End-to-End Network Delay Guarantees for Real-Time Systems using SDN

We propose a novel framework that reduces the management and integration overheads for real-time network flows by leveraging the capabilities (especially global visibility and management) of software-defined networking (SDN) architectures. Given the specifications of flows that must meet hard real-time requirements, our framework synthesizes paths through the network and associated switch configurations - to guarantee that these flows meet their end-to-end timing requirements. In doing so, our framework makes SDN architectures "delay-aware" - remember that SDN is otherwise not able to reason about delays. Hence, it is easier to use such architectures in safety-critical and other latency-sensitive applications. We demonstrate our principles as well as the feasibility of our approach using both - exhaustive simulations as well as experiments using real hardware switches.

==> For arxiv/Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> For arxiv/abstract.tex <==
\begin{abstract}
%Real-time systems (RTS) require end-to-end delay guarantees on delivery of
%network packets. Traditional approaches for providing such guarantees
%for mission critical applications often require the use of expensive
%custom built hardware and software resources. 

We propose a novel framework that reduces the management and integration
overheads for real-time network flows by leveraging the capabilities
(especially global visibility and management) of software-defined
networking (SDN) architectures. Given the specifications of flows that
must meet hard real-time requirements, our framework synthesizes paths
through the network and associated switch configurations -- to
guarantee that these flows meet their end-to-end timing requirements.
In doing so, our framework makes SDN architectures ``delay-aware'' -- remember
that SDN is otherwise not able to reason about delays. Hence, it
is easier to use such architectures in safety-critical and other latency-sensitive
applications. We demonstrate our principles as well as the feasibility of our approach using
both -- exhaustive simulations as well as experiments using real
hardware switches.

%%%%%%%%%%%%%%% RBB: Commented out on  1st May%%%%%%%%%%%%%%%%%%%%%%%%
% We propose a novel framework that reduces the management and integration overheads for
% real-time network flows by leveraging the capabilities (especially
% global visibility and management) of software-defined networking (SDN)
% architectures. Hence, given the specifications of flows that must meet
% hard real-time requirements, our framework synthesizes paths through
% the network and associated switch configurations -- to guarantee that
% these flows meet their end-to-end timing requirements.  On the other
% hand, current SDNs are not able to reason about delays (especially across the
% network). Hence our work also contributes to making such architectures
% ``timing-aware'' so that it is easier to use SDNs in safety-critical
% and other latency-sensitive applications. We demonstrate the
% feasibility of our approach using both -- exhaustive simulations as well
% as experiments using real hardware switches.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%the switch configuration for each flow that enables it to meet its bandwidth and delay requirements. Our empirical evaluation using controlled experiments on both physical and emulated networks connected in a variety of random topologies shows that each flow always meets both its bandwidth and percentile delay requirements.
%
\end{abstract}


==> For arxiv/algorithm_mcp.tex <==
\begin{algorithm}[t]

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}
\renewcommand\algorithmiccomment[1]{%
 {\it /* {#1} */} %
}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    
\renewcommand{\algorithmicforall}{\textbf{for each}}

\begin{algorithmic}[1]
\begin{footnotesize}
\Require The network $N (V,E)$, source $s$, destination $t$, constraints on links $W_1 = [w_1(u,v)]_{\forall(u,v) \in E}$ and $W_2 = [w_2(u,v)]_{\forall(u,v) \in E}$, and the bounds on the constraints $C_1  \in \mathbb{R}^+$ and $C_2 \in \mathbb{R}^+$ for the path from $s$ to $t$.
   \Ensure The path $\mathcal{P}^*$ if there exists a solution (\eg $W_1(\mathcal{P^*}) \leq C_1$ and $W_2(\mathcal{P^*}) \leq C_2$), or $\mathsf{False}$ otherwise.

\vspace{0.8em}

\Function{$\mathtt{MCP\_HEURISTIC}$}{$N, s, t, W_1, W_2, C_1, C_2$}
    \State \Comment{Initialize local variables}
  
    
    \State $d[v, i] := \infty, \pi[v, i] := NULL$, ~ $\forall v \in V$,~ $\forall i \in [0, C_2] \wedge i \in \mathbb{Z}$
    \State $d[s, i] := 0$~ $\forall i \in [0, C_2] \wedge i \in \mathbb{Z}$
    \State \Comment{Estimate path}
      \For{$i \in |V|-1$}
    	\ForAll{$j \in [0,C_2] \wedge j \in \mathbb{Z}$}
    		\ForAll{edge $(u,v) \in E$}
    			\State $j' := j + w_2(u,v)$
                \If {$j' \leq C_2$ \textbf{ and } $d[v, j'] > d[u, j] + w_1(u,v)$}
	               \State \Comment{Update estimation}
                	\State $d[v, j'] := d[u, j] + w_1(u,v)$  
                    \State $\pi[v, j'] := u$ ~\Comment{Store the possible path}
                \EndIf
	    	\EndFor
	    \EndFor
    \EndFor
    \State \Comment{Check for solution}
    \If{$d[t, i] \leq C_1 \textrm{ for } \exists i \in [0, C_2] \wedge i \in \mathbb{Z}$ }
    \State \Comment{Solution found, obtain the path by backtracking}
    
    \State $\mathcal{P} := $ \O, $done := \mathsf{False}$, $currentNode := t$ %\Comment{Initialize variables}
    \State \Comment{Find the path from $t$ to $s$}
    
    \While{\textbf{not} $done$} 
    	\ForAll{$j \in [0,C_2] \wedge j \in \mathbb{Z}$}
        	\If {$\pi[currentNode, j]$ \textbf{not}  $NULL$}                    			\State  %$path.\textrm{append}(currentNode)$
            add $currentNode$ to $\mathcal{P}$
            \If {$currentNode = s$} 
            \State $done := \mathsf{True}$ \Comment{Backtracking complete}
            \Break
            \EndIf
            %\Else
            \State \Comment{Search for preceding hop}
			\State $currentNode := \pi[currentNode, j]$ 
            \Break
            \EndIf
            
     
            
        \EndFor
    \EndWhile
    \State \Comment{Reverse the list to obtain a path from $s$ to $t$}
    \State $\mathcal{P}^*$ := \textrm{reverse}($\mathcal{P}$) 
    \State \Return $\mathcal{P}^*$
    \Else
    \State \Return $\mathsf{False}$ \Comment{No Path found that satisfies $C_1$ and $C_2$}
    \EndIf

\EndFunction

\end{footnotesize}

\end{algorithmic}
\caption{Multi-constraint Path Selection}
\label{alg:mcp_org}
\end{algorithm}
%\vspace{-0.2in}


==> For arxiv/algorithm_path.tex <==
\begin{comment}

\begin{algorithm}[t]

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}
\renewcommand\algorithmiccomment[1]{%
 {\it /* {#1} */} %
}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    
\renewcommand{\algorithmicforall}{\textbf{for each}}

\begin{algorithmic}[1]
\begin{footnotesize}
\Require The network $N (V,E)$, Set of flows $F$, delay and bandwidth utilization constraints on links  $\mathfrak{D}_k = [\mathfrak{D}_k(u,v)]_{(u,v) \in E}$ and $\mathfrak{B}_k = [\mathfrak{B}_k(u,v)]_{(u,v) \in E}$, for each flow $f_k \in F$, respectively, and the delay and bandwidth bounds $D_k  \in \mathbb{R}^+$ and $\widehat{B}_k \in \mathbb{R}^+$ $\forall f_k \in F$.
   \Ensure The path vector $\boldsymbol{\mathcal{P}} = [\mathcal{P}_k]_{\forall f_k \in F}$  where $\mathcal{P}_k$ is the path if the delay and bandwidth constraints (\eg $\mathfrak{D}_k(\mathcal{P}_k) \leq D_k$ and $\mathfrak{B}_k(\mathcal{P}_k) \leq \widehat{B}_k$) are satisfied for $f_k$, or $\mathsf{False}$ otherwise. 
\vspace{0.2em}
	%\State dd
%\State Solve \textrm{MCPS}($N, s_k, t_k, $)
\State \Return $path$

\end{footnotesize}
\end{algorithmic}
\caption{Obtain Path Considering Delay and Bandwidth Constraints}
\label{alg:mcp_path_delay_bw}
\end{algorithm}

\end{comment}


\begin{algorithm}[ht]

\newcommand{\algorithmicbreak}{\textbf{break}}
\newcommand{\Break}{\State \algorithmicbreak}
\renewcommand\algorithmiccomment[1]{%
 {\it /* {#1} */} %
}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
    \renewcommand{\algorithmicensure}{\textbf{Output:}}
    
\renewcommand{\algorithmicforall}{\textbf{for each}}

\begin{algorithmic}[1]
\begin{footnotesize}
\Require The network $N (V,E)$, set of flows $F$, delay and bandwidth utilization constraints on links  $\mathfrak{D}_k = [\mathfrak{D}_k(u,v)]_{\forall(u,v) \in E},~ \widetilde{\mathfrak{D}}_k = [\widetilde{\mathfrak{D}}_k(u,v)]_{\forall(u,v) \in E}$ and $\mathfrak{B}_k = [\mathfrak{B}_k(u,v)]_{\forall(u,v) \in E},~ \widetilde{\mathfrak{B}}_k = [\widetilde{\mathfrak{B}}_k(u,v)]_{\forall(u,v) \in E}$, for each flow $f_k \in F$, respectively, and the delay and bandwidth bounds $D_k  \in \mathbb{R}^+$ and $\widehat{B}_k \in \mathbb{R}^+$, respectively, and positive constant $X_k \in \mathbb{Z}$, $\forall f_k \in F$.
   \Ensure The path vector $\boldsymbol{\mathcal{P}} = [\mathcal{P}_k]_{\forall f_k \in F}$  where $\mathcal{P}_k$ is the path if the delay and bandwidth constraints (\eg $\mathfrak{D}_k(\mathcal{P}_k) \leq D_k$ and $\mathfrak{B}_k(\mathcal{P}_k) \leq \widehat{B}_k$) are satisfied for $f_k$, or $\mathsf{False}$ otherwise. 
\vspace{0.2em}

\ForAll{$f_k \in F$ (starting from higher to lower priority)} 
	\State \Comment{Relax bandwidth constraint and solve}
	\State Solve $\mathtt{MCP\_HEURISTIC}$($N, s_k, t_k, \mathfrak{D}_k, \widetilde{\mathfrak{B}}_k, D_k, X_k$) by using Algorithm \ref{alg:mcp_org}
    \If {$\mathsf{SolutionFound}$}~~
    \Comment{Path found for $f_k$}
      \State \Comment{Add path to the path vector $\boldsymbol{\mathcal{P}}$}
    \State $\mathcal{P}_k := \mathcal{P}^*$ where $\mathcal{P}^*$ is the solution obtained by Algorithm \ref{alg:mcp_org}
    \Else
    	\State \Comment{Relax delay constraint and try to obtain the path}
    \State Solve $\mathtt{MCP\_HEURISTIC}$($N, s_k, t_k, \widetilde{\mathfrak{D}}_k, \mathfrak{B}_k, X_k, \widehat{B}_k$) by using Algorithm \ref{alg:mcp_org}
        \If {$\mathsf{SolutionFound}$}
        \State \Comment{Path found by relaxing delay constraint}
    \State $\mathcal{P}_k := \mathcal{P}^*$ 
    \Comment{Add path to the path vector}
    \State \Comment{Update remaining available bandwidth} 
    \State $B_e(u,v) := B_e(u,v) - B_k, ~\forall (u,v) \in \mathcal{P}_k$ %~~\Comment{Update remaining available bandwidth}
    %\Comment{Path found by relaxing delay constraint} %where $\mathcal{P}^*$ is the solution obtained by \textrm{MCPS}($N, s_k, t_k, \widetilde{\mathfrak{D}}_k, \mathfrak{B}_k, X_k, \widehat{B}_k$)
    	\Else
        	\State $\mathcal{P}_k := \mathsf{False}$ ~~\Comment{Unable to find any path for $f_k$}
		\EndIf
    \EndIf
\EndFor

\end{footnotesize}


\end{algorithmic}
\caption{Layout Path Considering Delay and Bandwidth Constraints}
\label{alg:mcp_path_delay_bw}
\end{algorithm}
%\vspace{-0.15in}



==> For arxiv/approach.tex <==
\section{Path Layout: Overview and Solution}
%\section{Path Layout}
\label{sec:approach}
%\subsection{Path Layouts}
% \begin{itemize}
% \item Multi-constraint paths formulation
% \item Network calculus, Queueing theory(??) to get the upper bound
% \end{itemize}

%\subsubsection{Multi-constraint paths formulation}

% The first constraint in the MCP problem is the delay constraint. In the constraint $w_1(p)< c_1$, $c_1$ is the delay requirement of a flow given to us and $w_1(p)$ is the summation of delays of links in the path $p$. 

We now present a more detailed version of the problem (composing
paths that meet end-to-end delay constraints for critical real-time flows) and
also an overview of our solution.

\subsubsection*{Problem Overview}

Let $\mathcal{P}_k$ be the path from $s_k$ to $t_k$ for flow $f_k$ that needs
to be determined. Let $\mathfrak{D}(u, v)$ be the delay incurred on the edge
$(u,v) \in E$. 
%Assuming that propagation delays are negligible compared to the delays at the switch ports, 
The total delay for $f_k$ over the path $\mathcal{P}_k$ is  given by
\begin{equation}
%$
\mathfrak{D}_k(\mathcal{P}_k) = \sum_{(u,v) \in \mathcal{P}_k} \mathfrak{D}(u, v).
%$
\end{equation}
Therefore we define the following constraint on end-to-end delay for the flow $f_k$ as
\begin{equation} \label{eq:delay_con}
\mathfrak{D}_k(\mathcal{P}_k) \leq D_k.
\end{equation}

% \todo[inline]{Note that the end-to-end delay for a flow over a path has four delay components: 1) processing time of a packet at a switch 2) propagation on physical link, 3) serial transmission of packet over a physical link, and 4) queuing at the ingress/egress port of a switch. As discussed in the Section\ref{sec:system_model}, we use separate queue for each flow with assigned required rate. In the end-to-end delay, we consider queuing delay as negligible. Obtaining/calculating the values of other three components of delay is discussed in the evaluation section.} 



Note that the end-to-end delay for a flow over a path has following delay components: 
%\begin{inparaenum}[1)]
\ca processing time of a packet at a switch,
\cb propagation on the physical link,
\cc transmission of packet over a physical link, and
\cd queuing at the ingress/egress port of a switch.
%\end{inparaenum}
As discussed in the Section \ref{sec:system_model}, we use separate queues for
each flow with assigned required rates. We also overprovision the bandwidth
for such flows so that critical real-time flows do not experience queueing delays.
Hence, we consider queuing delays to be negligible. We discuss how to obtain 
the values of other components of delay in Appendix \ref{subsec:delay_cal}.

The second constraint that we consider in this work is {\em bandwidth utilization}, that
for an edge $(u,v)$ for a flow $f_k$, can be defined as:  
\begin{equation}
\mathfrak{B}_{k}(u,v) = \frac{B_k}{B_e(u,v)}
\end{equation}
where $B_k$ is the bandwidth requirement of $f_k$ and $B_e(u,v)$ is total bandwidth of an edge $(u,v) \in E$.
Therefore, bandwidth utilization over a path ($\mathcal{P}_k$), for a flow $f_k$ is defined as:  
\begin{equation}
	\mathfrak{B}_k(\mathcal{P}_k) = \sum_{(u,v)\in \mathcal{P}_k} \mathfrak{B}_{k}(u,v).
\end{equation}
Note that the bandwidth utilization over a path $\mathcal{P}_k$ for flow  $f_k$ is bounded by
\begin{equation}
  \mathfrak{B}_k(\mathcal{P}_k) \leq \max_{(u,v) \in E} \mathfrak{B}_{k}(u,v) |V|.
\end{equation}
% \begin{equation}
% \min_{(u,v) \in E} \mathfrak{B}_{k}(u,v) |V| <  \mathfrak{B}_k(\mathcal{P}_k) \leq \max_{(u,v) \in E} \mathfrak{B}_{k}(u,v) |V|.
% \end{equation}
where $|V|$ is the cardinality of a set of nodes (ports) in the topology $N$.
Therefore in order to ensure that the bandwidth requirement $B_k$ of the flow $f_k$ is guaranteed, it suffices to consider the following constraint on bandwidth utilization
\begin{equation} \label{eq:bw_con}
\mathfrak{B}_k(\mathcal{P}_k) \leq \widehat{B}_k
\end{equation}
where $\widehat{B}_k = \max\limits_{(u,v) \in E} \mathfrak{B}_{k}(u,v) |V|$
\begin{remark}
The selection of an optimal path for each flow $f_k \in F$ subject to delay and
bandwidth constraints in Eq. (\ref{eq:delay_con}) and (\ref{eq:bw_con}),
respectively can be formalized as a multi-constrained path (MCP) problem that
is known to NP-complete \cite{mcp_np_hard1}. 
\end{remark}

Therefore we extend a polynomial-time heuristic similar to that presented in
literature\cite{mcp_klara}. The key idea is to \textit{relax}
one constraint (\eg delay or bandwidth) at a time and try to obtain a solution.
If the original MCP problem has a solution, one of the relaxed versions of the
problem will also have a solution \cite{mcp_klara}. In what follows, we briefly
describe the polynomial-time solution for the path layout problem.

\subsubsection*{Polynomial-time Solution to the Path Layout Problem}

Let us represent the delay and bandwidth constraint as follows
\begin{align}
\widetilde{\mathfrak{D}}_k(u,v) &= \left\lceil \frac{X_k \cdot \mathfrak{D}(u,v)}{D_k} \right\rceil \label{eq:delay_relax} \\
\widetilde{\mathfrak{B}}_k(u,v) &= \left\lceil \frac{X_k \cdot \mathfrak{B}_k(u,v)}{\widehat{B}_k} \right\rceil \label{eq:bw_relax}
\end{align}
where $X_k$ is a given positive integer. For instance, if we relax the bandwidth constraint (\eg represent $\mathfrak{B}_k(\mathcal{P}_k)$ in terms of $\widetilde{\mathfrak{B}}_k(\mathcal{P}_k) = \sum_{(u,v)\in \mathcal{P}_k} \widetilde{\mathfrak{B}}_{k}(u,v)$), Eq. (\ref{eq:bw_con}) can be rewritten as
\begin{equation}
%$
\widetilde{\mathfrak{B}}_k(\mathcal{P}_k) \leq X_k.
%$ 
\end{equation}
Besides, the solution to this relaxed problem will also be a solution to the
original MCP \cite{mcp_klara}. Likewise, if we relax the delay constraint, Eq.
(\ref{eq:delay_con}) can be rewritten as 
\begin{equation}
\widetilde{\mathfrak{D}}_k(\mathcal{P}_k) = \sum_{(u,v)\in \mathcal{P}_k} \widetilde{\mathfrak{D}}_{k}(u,v) \leq X_k.
\end{equation}

Let the variable $d_k[v, i]$ preserve an \textit{estimate} of the path from
$s_k$ to $t_k$ for $\forall v \in V$, $i \in \mathbb{Z}^+$ (refer to
Algorithm \ref{alg:mcp_org}). There exists a solution (\eg a path
$\mathcal{P}_k$ from $s_k$ to $t_k$) if \textit{any} of the two conditions is
satisfied when the \textit{original MCP problem is solved by the heuristic}.
\begin{itemize}
\item \textit{When the bandwidth constraint is relaxed:} The delay and (relaxed) bandwidth constraints, \eg $\mathfrak{D}_k(\mathcal{P}_k) \leq D_k$ and $\widetilde{\mathfrak{B}}_k(\mathcal{P}_k) \leq X_k$ are satisfied if and only if $$d_k[t, i] \leq D_k, ~~ \exists i \in [0, X_k] \wedge i \in \mathbb{Z}.$$

\item \textit{When the delay constraint is relaxed:} The (relaxed) delay and bandwidth constraints, \eg $\widetilde{\mathfrak{D}}_k(\mathcal{P}_k) = \sum_{(u,v)\in \mathcal{P}_k} \widetilde{\mathfrak{D}}_{k}(u,v) \leq X_k$ and $\mathfrak{B}_k(\mathcal{P}_k) \leq \widehat{B}_k$ are satisfied if and only if $$d_k[t, i] \leq X_k, ~~ \exists i \in [0, \widehat{B}_k] \wedge i \in \mathbb{Z}.$$
\end{itemize}


%\subsubsection{Analysis of the Proposed Solution}

% \subsubsection{Algorithm Development and Analysis}

\section{Algorithm Development} 
\label{sec:algo}

\subsection{Path Layout}

Our proposed approach is based on a polynomial-time solution to the MCP problem presented in literature \cite{mcp_klara}. Let us consider $\mathtt{MCP\_HEURISTIC}$($N, s, t, W_1, W_2, C_1, C_2$), an instance of polynomial-time heuristic solution to the MCP problem that finds a path $\mathcal{P}$ from $s$ to $t$ in any network $N$, satisfying constraints $W_1(\mathcal{P}) \leq C_1$ and $W_2(\mathcal{P}) \leq C_2$. \input{mcp_base}


\input{algorithm_path}

%Based on this MCP abstraction, the proposed path selection scheme  considering delay and bandwidth constraints (\textbf{Algorithm \ref{alg:mcp_path_delay_bw}}) works as follows. 

%Based on this MCP abstraction, we developed a path selection scheme  considering delay and bandwidth constraints (Algorithm \ref{alg:mcp_path_delay_bw}) that works as follows.

For each flow $f_k \in F$, starting with highest (\eg the flow with tighter delay requirement) to lowest priority, we first keep the delay constraint unmodified and relax the bandwidth constraint by using Eq. (\ref{eq:bw_relax})  and solve $\mathtt{MCP\_HEURISTIC}$($N, s_k, t_k, \mathfrak{D}_k, \widetilde{\mathfrak{B}}_k, D_k, X_k$) (Line 3) using Algorithm \ref{alg:mcp_org}. If there exists a solution, the corresponding path $\mathcal{P}_k$ is assigned for $f_k$ (Line 6). However, if relaxing bandwidth constraint is unable to return a path, we further relax delay constraint by using Eq. (\ref{eq:delay_relax}), keeping bandwidth constraint unmodified and solve $\mathtt{MCP\_HEURISTIC}$($N, s_k, t_k, \widetilde{\mathfrak{D}}_k, \mathfrak{B}_k, X_k, \widehat{B}_k$) (Line 9). If the path is not found after \textit{both} relaxation steps, the algorithm returns False (Line 14) since it is not possible to assign a path for $f_k$ such that both delay and bandwidth constraints are satisfied. Note that the heuristic solution of the MCP depends of the parameter $X_k$. From our experiments we find that if there exists a solution, the algorithm is able to find a path as long as $X_k \geq 10$.


%\subsubsection{Complexity Analysis}
\subsection{Complexity Analysis}

Note that Line 8 in Algorithm \ref{alg:mcp_org} is executed at most $(C_2 + 1)(V-1)E$ times. Besides, if there exists a path, the worst-case complexity to extract the path is $|\mathcal{P}| C_2$. Therefore, time complexity of Algorithm \ref{alg:mcp_org} is $O(C_2 (V E + |\mathcal{P}|)) = O(C_2 V E)$. Hence the worst-case complexity (\eg when both of the constraints need to be relaxed) to execute Algorithm \ref{alg:mcp_path_delay_bw} for each flow $f_k \in F$ is $O((X_k + \widehat{B}_k )V E)$. 


%The proposed heuristic as summarized i
%\end{equation}



% Bandwidth utilization of an edge (link) for a flow, $f$, can be defined as:  
% \begin{equation}
% BU(f,l) = \frac{Br(f)}{B(l)}
% \end{equation}
% where $Br(f)$ is the bandwidth requirement of $f$ and $B(l)$ is total bandwidth of a link $l$.
 
% Bandwidth utilization over a path($p$), for a flow $l$ is defined as:  
% \begin{equation}
% BU(f,p) = \sum_{l\in p} (BU(f,l))
% \end{equation}

 
\begin{comment}

 
How does the bandwidth requirement of a flow provided to us translate to bandwidth utilization bound in MCP?
 \begin{itemize}
\item Controller has all information on the bandwidth of each link and the topology information.
\item Controller finds the max hops a path can have between a source and destination (loop-free), say $h_{max}$. May use minimum spanning tree or any other existing efficient algorithm. 
 \item Then the cost (bandwidth utilization) bound will be:
 \begin{equation}
 \min_{l\in E} BU(f,l))*h_{max} < w_2(p) \le \max_{l\in E} BU(f,l)*h_{max}
 \end{equation}
 \item If for a flow’s cost bound exceeds $h_{max}$, then bound should be $w_2(p)<= h_{max}$
\end{itemize}

Now, to compute new weight function $w_2^{'}$, choose $x$ as large enough so that the condition stated in Theorem 3 of the Klara's paper is satisfied. An worst case example could be to choose $x=10|V|$ or $w_2(p)<0.92c_2$.

$x$ depends on the topology. So we may need to run the experiment several times before deciding on a value.

Section 2.3 of the Klara's paper describes the steps to solve MCP and when to use EDSP/EBF algorithm
\end{comment}





==> For arxiv/background.tex <==
\section{Background}
\label{sec:background}

\subsubsection{The Software Defined Networking Model}

% The communication network orchestrates packet delivery among all network devices by using packet headers. Its configuration drives the two components of the networking software: control and data planes. The control plane decides what packet forwarding and header transformations need to occur at network devices, while the data plane performs the actual actions on packets. 
In traditional networking architectures, control and data planes coexist on
network devices. SDN architectures simplify access the system by logically centralizing the control-plane state in a
\textit{controller} (see Figure~\ref{fig:sdn_model}). This programmable and
centralized state then drives the network devices that perform homogeneous
forwarding plane functions \cite{casado2009rethinking} and can be modified to
control the behavior of the SDN in a flexible manner. 

\begin{figure}[ht!]
\centering
\vspace*{-1em}
\includegraphics[width=2.2in]{graphics/system_architecture.png}
\caption{An SDN with a six switch topology. Each switch also connects to the controller via a management port (not shown). The QoS Synthesis module (Section \ref{sec:implementation}) synthesizes flow rules by using the northbound API.}
\label{fig:sdn_model}
\vspace{-0.2in}
\end{figure} 

In order to construct a logically centralized \textit{state} of the SDN system, the
controller uses management ports to gauge the current topology and
gather data-plane state from each switch. This state is then made available
through a \textit{northbound} API to be used by the applications. An
application (\eg our prototype proposed in this paper) uses this API to
obtain a snapshot of the SDN state. %and constructs a model to predict the behavior of the SDN. 
This state also includes the network topology.

\subsubsection{The Switch}

An SDN switch consists of table processing pipeline and a collection of
physical \textit{ports}. Packets arrive at one of the ports and they are
processed by the pipeline made up of one or more flow tables. Each flow table
contains \textit{flow rules} ordered by their priority. Each flow rule
represents an atomic unit of decision-making in the control-plane. During the
processing of a single packet, \textit{actions} (\eg decision-making entities)
can modify the packet, forward it out of the switch or drop it. 

When a packet arrives at a switch, it is compared with flow rules in one or
more flow table pipelines. In a given table, the contents of the packet header
are compared with the flow rules in decreasing order of rule priority. When
a matching flow rule is found, the packet is assigned a set of
actions specified by the flow rule to be applied at the end of table processing
pipeline. Each flow rule comprises of two parts:

%apply to the given rule
\begin{itemize}
\item \textbf{Match}: is set of packet header field values that a given flow rule applies to. Some are characterized by single values (\eg VLAN ID: 1, or TCP Destination Port: 80), others by a range (\eg Destination IP Addresses: 10.0.0.0/8). If a packet header field is not specified then it is considered to be a wild card.

\item \textbf{Instructions Set}: is a set of actions applied by the flow rule to a matching packet. The actions can specify the egress port ($\mathsf{Output Port}$) for packets matching the rule. Furthermore, in order to make the appropriate allocation of bandwidth for the matching packets, the OpenFlow \cite{specification20131} specification  provides two mechanisms:

\begin{itemize}

\item \textbf{Queue References}: Every OpenFlow switch is capable of providing isolation to traffic from other flows by enqueuing them on separate queues on the egress port. Each queue has an associated QoS configuration that includes, most importantly, the service rate for traffic that is enqueued in it. The OpenFlow standard itself does not provide mechanisms to configure queues, however, each flow rule can refer to a specific queue number for a port, besides the $\mathsf{Output Port}$.

\item \textbf{Meters}: Beyond the isolation provided by using queues, OpenFlow switches are also capable of limiting the rate of traffic in a given network flow by using objects called meters. The meters on a switch are stored in a meter table and can be added/deleted by using messages specified in OpenFlow specification. Each meter has an associated metering rate. Each flow rule can refer to only a single meter. 

\end{itemize}

\end{itemize}



==> For arxiv/concl.tex <==
\section{Conclusion}
\label{sec:concl}

With the proliferation of commercial-off-the-shelf (COTS) components, 
designers are exploring new ways of using them, even in critical systems
(such as RTS).
Hence, there is a need to understand the inherent trade-offs (less customization)
and advantages (lower cost, scalability, better support and more choices)
of using COTS components in the design of such systems. In this paper, we
presented mechanisms that provide end-to-end delays for critical traffic
in real-time systems using COTS SDN switches. Hence, future RTS can be
better managed, less complex (fewer network components to deal with) and
more cost effective. 


==> For arxiv/delay_calculations.tex <==

%\subsection{Delay Calculations} 
%\label{subsec:delay_cal}

Remember that some of the critical pieces of information that is required for
any such scheme (for ensuring end-to-end delays) is a measure of the delays
imposed by the various components in the system. Hence, we need to obtain
network delays at each link. We use these estimated delays as the weights of
edges of the network graph in the MCP algorithm within the experimental setup to
obtain solutions. As discussed earlier, we assume zero queuing delay. The
transmission and propagation delays are a function of the physical properties
of the network topology. However, the processing delay of an individual switch
for a single packet can be empirically obtained. Here we describe our method to
obtain upper-bounds on each of these delay components.

\subsection*{Estimation of Propagation Delay}
The transmission delay is calculated as $\frac{\text{packet
length}}{\text{bandwidth allocated}}$. In our experiments we assume the packet
length is [25, 125] bytes and the maximum bandwidth can be allocated allocated
in a specific link is 10 Mbps. Then transmission delay on that link will be
upper bounded by $\frac{125 \times 8~\text{bits}}{10~ \text{Mbps}}$ = 100
$\mu$s. Therefore delay of the edge, \ie $\mathfrak{D}_k(u, v)$, $\forall (u,v)
\in E$ is upper bounded by 3.6+0.505+100 $\approx$ 105 $\mu$s.

\subsection*{Estimation of Transmission Delay}
The propagation delay depends on the physical link length and propagation speed
in the medium. In the physical media, the speed varies .59$c$ to .77$c$ \cite{prop_delay} where
$c$ is speed of light in vacuum. We assume that the length of any link in the
network to be no more that 100 $m$. Therefore the propagation delay is upper bounded
by $\frac{100 \rm m}{0.66 \times 3 \times 10^6} = 505$ ns in fiber-link media. 

\subsection*{Estimation of Processing Delays}

We experimented with a software switch, Open vSwitch (OVS) \cite{ovs} version
2.5.90 to compute the time it takes to process a packet within its data path.
Since this timing information is platform/architecture dependent, we summarized
the hardware information of our experimental platform in Table
\ref{tab:delay_param}. 

\input{delay_hw_info}

\begin{figure}[H]
\centering
\includegraphics[width=2.7in]{graphics/ovs_arch_mod}
\caption{Interaction of kernel timing module with the existing OVS architecture.}
\label{fig:ovs-arch-mod}
\end{figure}

We modified the kernel-based OVS data path module called
\texttt{openvswitch.ko} to measure the time it takes for a packet to move from
an ingress port to an egress port. We used \texttt{getnstimeofday()} for
high-precision measurements. We also developed a kernel module called
\texttt{netlinkKernel.ko} that copies the shared timing measurement data
structure between the two kernel modules and communicates it with a user space
program called \texttt{netlinkUser}. We disabled scheduler preemptions in the
\texttt{openvswitch.ko} by using the system calls \texttt{get\_cpu()} and
\texttt{put\_cpu()}, hence the actual switching of the packets in the data path
is not interfered by the asynchronous communication of these measurements by
\texttt{netlinkKernel.ko}. We also used compilation flags to ensure that
\texttt{openvswitch.ko} always executes on a specified, separate, processor
core of its own (with no interference from any other processes, both from the
user space or the operating system). For fairness in the timing measurements
and stabilized output, we disabled some of the Linux background processes (\eg
SSH server, X server) and built-in features (\eg CPU frequency scaling). Figure
\ref{fig:ovs-arch-mod} illustrates the interaction between the modified kernel
data path and our user space program.



We used the setup described above with Mininet and Ryu Controller. We evaluated
the performance and behavior of OVS data path under different flows, network
typologies and packet sizes. We executed several runs of the experiment with UDP
traffic with different packet sizes (100, 1000, 1600 bytes). We observed that
average processing time for a single packet within the software switch lies
between 3.2 $\mu$s to 4.1 $\mu$s with average being 3.6 $\mu $s and standard
deviation being 329.61 ns. These were the values that were used in the path 
allocation calculations.


==> For arxiv/delay_hw_info.tex <==
\begin{table}[!htb]
\renewcommand{\arraystretch}{1.2}
\caption{Hardware used in Timing Experiments}
\label{tab:delay_param}
\centering
%\begin{tabular}{c||p{5.9cm}}
\begin{small}
\begin{tabular}{p{3.20cm}||p{4.30cm}}
\hline %\\
\bfseries Artifact & \bfseries Info\\
\hline\hline
Architecture &              i686 \\
CPU op-modes &       32-bit, 64-bit \\
Number of CPUs &                     4 \\
%On-line CPUs list &    0-3 \\
Threads per core &     2 \\
Cores per socket &     2 \\
CPU family &               6 \\
L1d and L1i cache &              32K \\
L2 and L3 cache &               256K and 3072K, respectively \\
\hline
\end{tabular}
\end{small}
\end{table}

==> For arxiv/design.tex <==
\section{Design}
\label{sec:design}

% We consider following broad classes of requirements:

% Class 1: perflow, hard real time guarantee, control applications in avionics (AFDX)

% class 2: Fairness and soft real time, avionics infrastructure,  autopilot few miliseconds delay, (papers?)
% class 3: entertainment systems, (everything else)

There are three elements of the QoS Synethsis that we tackle separately:

1. Admission Control (Book-keeping, incremental addition of flows as system evolves)

2. Intent Generation (Graph Theory Aborescenes): 

3. QoS Paramater for Intents (Which queue a given intent uses at a switch, what the rate of the queue is set to, what queueing discipline is applied)



We take as input the set of flows that require to be synthesized.

We then compute the following:

1. The ingress filtering rules keep applications honest and limit them at the ingress.

2. We compute rules at each individual switch that need to be installed in order for all the required flows to meet the guarantees.

3. We compute parameters such as traffic rates and the queuing discipline used by packet queues that are referred by the flow rules computed previously.

Each one of these is accomplished as following:

\subsection{Ingress Filtering}
\input{ingress_filtering}
\subsection{Rules Computation}
\subsection{Packet Queue Parameter Computation}




==> For arxiv/detailed_arch.tex <==
\section{Detailed Architecture}
\label{sec::detailed_arch}

We now present more details about our \SKM{}-based two-level monitoring
architecture. The overall process is presented in Figure 
\ref{fig::overall_process}. We first explain this high level flow
and then delve into the details in the following sections.

\subsection{\SKM{} Architecture Operations}
\label{subsec::skm_operations}

Consider the example of detecting problems in the system call table (presented
in Section \ref{subsec::example_use_cases}). To understand the sequence of operations in our system, we describe in detail each step shown in Figure~\ref{fig::overall_process}:
\begin{enumerate}
	\item The \SKMMan{} sends the command to check the system call table. This
		command is written in the secure memory that is part of the \SKMHW{}.
	\item The above process results in an inter-core interrupt that is handled
		by an interrupt handler on the monitored core.\footnote{We will use
		`monitored core', `application core' and `main core' interchangeable.}
		We implement an interrupt-service routine to handle this specific
		interrupt, {\tt skm\_ISR()}.
	\item The ISR calls into the \SKM{} ({\tt skm\_tasklet()}) that handles
		the command sent by the \SKMMan{}. The \SKM{} then determines what
		exact command was called (in this case it was instructed to copy
		the system call table). No entity on the main core (other than the 
		\SKM{}) can decipher the command because access to the secure memory 
		is restricted. 
	\item The tasklet calls the appropriate function to carry out the required task
		\ie gather the information requested by the \SKMMan{}.
	\item The function (e.g., to copy the system call table) carries out its
		operations by placing the required information in the secure
		memory of the \SKMHW{}. 
	\item The secure core receives an interrupt that the data it requested is
		now available in the secure memory. On receiving the interrupt, 
		the \SKMMan{} starts to read out the information from the secure memory 
		region and then sends it to the appropriate module in the secure 
		core that can analyze this information.
\end{enumerate}
The above process repeats for every command that is sent by the \SKMMan{} to the \SKM{}.
Let us now look at more of the details that enable the above process.


\subsection{\SKM{} Setup}
\label{subsec::skm_setup}

The \SKM{} is loaded onto the monitored core during the OS booting phase. As mentioned in the threat model, we make the assumption here that the system is in a clean state at boot time. For this, one can use a secure-boot mechanism such as IMA~\cite{sailer2004design}. 

\begin{figure}[tb]
   \centering
   \includegraphics[width=0.95\columnwidth]{Figures/registration.pdf}
   \caption{\SKM{} registration during secure boot}
   \label{fig::registration}
\end{figure}

The first task for the \SKM{} (during load time) is to request the \SKMMan{} to 
register it, \ie authenticate itself (Figure \ref{fig::registration}). 
For the \SKMMan{} to test the veracity of
the \SKM{} request for registration, it uses a hash of the \SKM{}'s {\tt .text} section.
The \SKMMan{} then compares this newly computed hash with the value that was
obtained at design time (and is stored in the secure core). We do not trust
the \SKM{} yet---hence, we do not wait for the \SKM{} to send its hash but rather
calculate it independently in the \SKMMan{}. This prevents the situation where
a malicious module could copy the \SKM{}'s hash and try to pass off as the
legitimate module.

The \SKMMan{} needs the following information about the \SKM{} to compute this
hash value: \ca the virtual base address, \cb the size of the {\tt .text}
section, \cc the page size and the \cd page table information---all for the
\SKM{}. In ARM processors, the last piece of information corresponds to the translation
table base register 0 ({\tt TTBR0}) that holds the physical address of the
first level translation table $0$.\footnote{Depending on the OS and the
system configuration, the translation table base register $1$ ({\tt TTBR1})
may also be required in addition to {\tt TTBR0}. In our implementation the
\SKMMan{} is provided with both {\tt TTBR0} and {\tt TTBR1}, which
does not change the authentication process} The \SKMMan{} then translates the 
{\tt .text} section of the \SKM{} as defined by the base (virtual) address and 
its size to a set of physical addresses that host the \SKM{} code.

As shown in Figure \ref{fig::registration}, the \SKMMan{} then calculates a
hash of the data stored in the pages that store the \SKM{} code using 
the \textsf{SHA-1} algorithm. If the newly computed hash matches
what was calculated before (\ie at the time the \SKM{} was developed) then
the \SKMMan{} registers the base address for the \SKM{}'s {\tt .text} section, 
its size and {\tt TTBR0} with the \SKMHW{}. From then on, the secure memory
in the \SKMHW{} can only be access by the monitored core when it is executing
code that is known to be part of the \SKM{}.

%\todo[inline]{The following paragraph somehow does not make sense
%to me -- Sibin.}
%\note If the physical addresses of the \SKM{} were provided to the \SKMMan{} during
%the registration process, then a malicious module can claim itself to be
%the \SKM{} by mapping its own virtual address information to the \SKM{}'s
%physical addresses. Thus, the malicious module would pass the authentication
%because the original \SKM{}'s hash will be used. It could then access the secure 
%memory since its virtual address is registered with the \SKMHW{}. Our approach 
%of transferring the responsibility of translating the virtual to physical 
%address mapping to the \SKMMan{} prevents such attacks because the addresses
%used for the authentication as well as checking the access to the secure
%memory are the same.


\subsection{Secure Memory and Access Control}
\label{subsec::secure_memory}

\begin{figure}[t] 
\centering
\includegraphics[width=1\columnwidth]{Figures/secure_memory.pdf}
\caption{Secure memory access control on the \SKMHW{}.}
\label{fig::secure_memory}
\end{figure}

The secure memory on the on-chip \SKMHW{} unit is a key component in our
architecture. This memory enables secure and trusted communication between the
\SKM{} and the \SKMMan{}. A `secure memory controller' (associated with the
\SKMHW{}) only allows instructions that are part of the \SKM{} to access this on-chip
memory, at least from the main core.\footnote{Of course, any process on the
secure core can access this secure memory---this is guaranteed by
checking if the access requests are coming from the secure core.} To
implement this type of `access control', we need to check {\em who is
executing} on the monitored core when a memory transaction is issued
for the secure memory. The \SKMHW{} accesses the program counter register
({\tt PC}) on the main core (a virtual address) as well as the {\tt
TTBR0} register. It then checks if
\ci the {\tt TTBR0} register matches the one registered by the \SKM{} (as 
explained in Section \ref{subsec::skm_setup}) and
\cii the value of the {\tt PC} register is within the {\tt .text} region
of the \SKM{}. This ensures that only \SKM{} can access the secure on-chip memory. If the memory
controller detects an illegal access attempt (\ie access by a process
different from the \SKM{} or instructions that lie outside its legitimate
range) then the \SKMHW{} raises an alert and notifies the \SKMMan{}. The latter
can then take appropriate actions to counter the problem. Figure 
\ref{fig::secure_memory} presents this process.
 
However, it is entirely likely that a smart adversary may have modified the
address mapping thus making it look like its own instructions that falls
within the allowed virtual address space now points to different physical
addresses (that actually hosts malicious code instead of the \SKM{}). Hence,
the above access control mechanism will fail to prevent the malicious code
from access the secure memory. To prevent such issues, we could check the
physical addresses of the instructions trying to access the on-chip memory
to see if it falls within the expected range (of the \SKM{}). However,
we avoid this option since it would involve an address translation each time
the secure memory is accessed---this would result in huge performance
overheads. Our solution (as will be elaborated in Section \ref{subsec::heartbeat})
is for the \SKMMan{} to \ca translate the \SKM{}'s {\tt .text}
section from virtual to physical addresses and \cb calculate the hash of the
resultant pages---following exactly the same process as the registration, only
done often during execution, not just at boot time.
As long as the resultant hash value matches the original we can be sure that
the \SKM{} has not been tampered with.\footnote{Of course, this does not eliminate
the possibility where a carefully constructed malicious module changes the
address mappings and restores it to the original between two hash check points.
However, regular hashing with random time intervals can significantly reduce
the possibility of success for such attempts.}

Because of this stringent access control for the secure memory, we 
may not be able to use some kernel library functions, \eg \textsf{printk}. This is
particularly true if the arguments for such library functions (a string
in this case) is stored in the secure memory since the program counter
for the library function will fall outside the acceptable range of the
\SKM{}'s {\tt .text} region. One way to get around this issue is to write a 
wrapper function in the \SKM{} that copies the required data to some part of
the main memory and then pass it to the required library functions. 
There will never be an instance when sensitive data is passed outside
of the \SKM{} (or the \SKMHW{} memory module).

\subsection{Heartbeat and \SKM{} Integrity Check}
\label{subsec::heartbeat}

As mentioned earlier, we need to periodically check if 
\ci the \SKM{}'s code has not been tampered with;
\cii the \SKM{} is actually starting up when it is commanded to do so by the \SKMMan{}
and finally, \ciii the \SKM{} responds to requests in a timely manner.
We have already discussed a technique to check for \ci -- periodically
hash the {\tt .text} region of the \SKM{} and check against previously stored
values. The issues of liveness of the \SKM{}, \viz~\cii and \ciii, require a
more active approach on behalf of the \SKMMan{}.

Our solution for this problem is to send out a special command, every once
in a while, to the \SKM{}. The \SKM{} should respond to this command right away.
This ensures that the \SKM{} has not be deactivated by an adversary. No other
process/code can respond to this command since the communication happens 
through the secure memory that has a form of access control implemented
on it (Section \ref{subsec::secure_memory}). When the special command is
sent to the \SKM{}, the \SKMMan{} starts a countdown timer ($500 ms$ in our experiments). If it 
does not receive the expected response from the \SKM{} then this is also 
indicative of an attack. The timer can be used for any/all commands that
the \SKMMan{} sends across -- if the responses/information does not start
arriving before the timer expires then the \SKMMan{} can raise an alert and
assume that the \SKM{} has been attacked.

Another precaution that we can take is to send out these heartbeat commands at {\em random} intervals so that an adversary 
cannot guess the pattern of checks by the \SKMMan{}.


\subsection{Inter-core Interrupts for Communication}
\label{subsec::interrupts}

As mentioned earlier, we use inter-core interrupts to initiate communications
between the main and secure cores. When the \SKMMan{} sends a command via the
secure memory, it results in an interrupt to the monitored core. This interrupt
is handled by the \SKM{}'s interrupt service routine. For the sake of efficiency,
we use the `tasklet' mechanism in Linux. The code in the tasklet
parses the command from the \SKMMan{}. It calls whatever functions that are
required (and part of the \SKM{}) to complete the task. The results of the operation(s)
are placed back into the secure memory region. This generates another inter-core
interrupt but this time on the secure core side. The \SKMMan{} handles this interrupt
and routes the information to the appropriate analysis module.

The tasklet on the \SKM{} is not synced with the interrupt service routines. There
is a small chance that some finite time passes between the ISR invoking the
tasklet and the latter being scheduled to run. Hence, an attacker may prevent
the tasklet from executing. Hence, as mentioned in Section
\ref{subsec::heartbeat} the \SKMMan{} uses a timeout mechanism. When a command is
sent, a countdown timer is started. The expiration of the time (before
receiving any results from the other side) is a strong indicator of the main
core (and the \SKM{} in particular) being under attack.

When an interrupt is raised and handled by the \SKM{}, the first
step taken by an ISR is to change the stack pointer (for a context switch). This
could result in problems if the main stack is attacked by the adversary. Hence, 
we allocate the stack for the \SKM{} in the secure on-chip memory. We change the
stack pointer every time (to a random part of the secure memory) the \SKM{} 
handles an interrupt.

Since we will place the ISR in the \SKM{}'s {\tt .text} section, any attempts by
the attacker to change the ISR will be detected by the mechanisms mentioned earlier.
If, on the other hand, the main core's interrupts are disabled (especially the
inter-core interrupts) then the timeout mechanism described earlier will detect it.


\subsection{Secure Memory and the \SKMMan{}}
\label{subsec::skmman_mem}

\begin{figure}[htb] 
\centering
\includegraphics[width=0.45\columnwidth]{Figures/secure_memory_map.pdf}
\caption{The secure memory map.}
\label{fig::secure_memory_map}
\end{figure}

To ensure the integrity of the \SKMMan{} we load its code onto a part of the
secure memory region as shown in Figure \ref{fig::secure_memory_map}. Hence,
an attacker that takes control of the main core cannot corrupt the \SKMMan{}. The
\SKM{}, on the other hand, will be loaded onto the main memory (along with the
rest of the kernel)---of course, we will monitor and protect the \SKM{}'s memory
region by the various mechanisms described in this section. 



\subsection{Implementation-Specific Assumptions}
\label{subsec::impl_assumptions}

% \todo[inline]{Collect assumptions here. -- Sibin.}

The primary assumption we make as part of designing this mechanism is that the \SKMMan{} has the ability to access any region in the main memory using physical addresses. Since the \SKMMan{} runs on the SecureCore, which satisfies this requirement, this is not a challenging assumption to discharge.

% \todo[inline]{Anything else in this section? Do we need more subsections here? -- Sibin.}

==> For arxiv/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

% \todo[inline]{1. Update the parameters that scales with the delay and bw requirements (e.g. 100 Mbps is much higher in 8 flows requires 5 Mbps -- not very utilized

% 2. How about delay if the links are used by other non-real time flows?

% 3. need to show the delay with and without our schemes

% 4. Describe more about the intents translate into controllers and integration with MCP and intents

% 5. Try and Test the ideas with HP switches.

% 6. make footnotes (2), (3) -- about openvswitch and ryu -- into references\\

% Notes from Meeting on 10/20:
% 1. How do we deal with the queueing delays in the switches? We need to explain the assumptions in the paper regarding this.

% 2. Can we try the multiple topologies on real switches?

% 3. Need a better writeup for how the path generation algorithm is evaluated and its corner cases.}

In this section, we evaluate our proposed solutions using the following
methods:
\ca an exploration of the design space/performance of the path layout 
algorithm in Section \ref{subsec:exp:synthetic}, and
\cb an empirical evaluation, using Mininet, that demonstrates the effectiveness
of our end-to-end delay guaranteeing mechanisms even in the presence of other
traffic in the network (Section \ref{subsec:exp:mininet}).
%We evaluate the performance of proposed approach with randomly generated
%synthetic networks (Section \ref{subsec:exp:synthetic}) as well as with
%Mininet topology and UDP traffic using SDN controllers and switches (Section
%\ref{subsec:exp:mininet}). 
The parameters used in the experiments are summarized in Table \ref{tab:ex_param}.

\input{experiment_param}

%\subsection{Experiment with Synthetic Network Topology} 
\subsection{Performance of the Path Layout Algorithms}
\label{subsec:exp:synthetic}

\subsubsection*{Topology Setup and Parameters} 
\label{sec:synthetic_setup}

In the first set of experiments we explore the design space (\eg feasible delay
requirements) with randomly generated network topologies and synthetic flows. For
each of the experiments we randomly generate a graph with 5 switches and
create $f_k \in [2, 20]$ flows. %Since we allocate each flow to individual queues, we limit the number of flows to $8$ -- the maximum allowable queues in many commercial switches\cite{?}. 
Each switch has 2 hosts connected to it. We
assume that the bandwidth of each of the links $(u,v) \in E$ is 10 Mbps 
%(\eg Fast Ethernet, IEEE 802.3u standard \cite{gigabit_ethernet}) 
(\eg IEEE 802.3t standard \cite{ethernet_standard}). 
%and %based on the discussion on Section \ref{subsec:delay_cal}, 
The link delays are 
randomly generated within [25, 125] $\mu$s (refer to Appendix \ref{subsec:delay_cal} for the calculation of link delay parameters). For each randomly-generated topology, 
we consider the bandwidth requirement as $B_k \in [1, 5]$ Mbps, $\forall f_k$.

\subsubsection*{Results}


\begin{figure}[!t]
\centering
\vspace*{-2em}
\includegraphics[width=3.3in]{graphics/schedulability}
\caption{Schedulability of the flows in different network topology. For each of the (delay-requirement, number-of-flows) pair (\eg $x$-axis and $y$-axis of the figure), we randomly generate 250 different topology. In other words, total 8 $\times$ 7 $\times$ 250 = 14,000 different topology were tested in the experiments.}
\label{fig:schedulabiliy}
\vspace{-0.2in}
\end{figure}

We say that a given network topology with set of flows is \textit{schedulable}
if all the real-time flows in the network can meet the delay and bandwidth
requirements. We use the \textit{acceptance ratio} metric ($z$-axis in
Fig.~\ref{fig:schedulabiliy}) to evaluate the schedulability of the flows. 
{\em The acceptance ratio is defined as the number of accepted topologies
(\eg the flows that satisfied bandwidth and delay constraints) over the total
number of generated ones}. To observe the impact of delay budgets in different
network topologies, we consider the end-to-end delay requirement $D_k,~ \forall
f_k \in F$ as a function of the topology. In particular, for each randomly
generated network topology $G_i$ we set the minimum delay requirement for the
highest priority flow as $D_{min} = \beta \delta_i$ $\mu$s, and increment it by
$\frac{D_{min}}{10}$ for each of the remaining flows. Here $\delta_i$ is the
diameter (\eg maximum eccentricity of any vertex) of the graph $G_i$ in the
$i$-th spatial realization of the network topology, $\beta =
\frac{D_{min}}{\delta_i}$ and $D_{min}$ represents $x$-axis values of
Fig.~\ref{fig:schedulabiliy}\footnote{Remember our ``delay-monotonic'' priority
assignment where flows with lower end-to-end delays have higher priority.}. 
For each (delay-requirement, number-of-flows) pair, we randomly generate 250 
different topologies and measure the acceptance ratios. As Fig.~\ref{fig:schedulabiliy} 
shows, stricter delay requirements (\eg less than 300 $\mu$s for a set of 20 flows) limit the 
schedulability (\eg only 60\% of the topology is schedulable). Increasing the
number of flows limits the available resources (\eg bandwidth) and thus the
algorithm is unable to find a path that satisfies the delay requirements of \textit{all}
the flows. 
%However from our experiments we find that, a network with the parameters specified in Section \ref{sec:synthetic_setup} can accommodate up to 8 flows as long as the delay requirement is not less than 500 $\mu$s.

\subsection{Experiment with Mininet Topology: Demonstrating that the End-to-End Delay Mechanisms Work} 
\label{subsec:exp:mininet}

\subsubsection*{Experimental Setup}

The purpose of the experiment is to evaluate whether our controller rules and
queue configurations can provide isolation guarantees so that the real-time flows can meet
their delay requirement in a practical setup. We evaluate the performance of
the proposed scheme using Mininet \cite{lantz2010network} (version 2.2.1) where switches are
configured using Open vSwitch \cite{ovs} (version 2.3.0). We use Ryu \cite{ryu}
(version 4.7) as our SDN controller. For each of the experiments we randomly
generate a Mininet topology using the parameters described in
Table \ref{tab:ex_param}.
%Section \ref{sec:synthetic_setup}.
%graph with 5 switches and create $f_k \in \lbrace 2, 4, 6, 8 \rbrace$ flows\footnote{Since we allocate each flows to individual queues, we limit the number of flows to 8, which is the maximum allowable queues in many commercial switches.}. We assume that the bandwidth of each of the links $(u,v) \in E$ is 10 Mbps %(\eg Fast Ethernet, IEEE 802.3u standard \cite{gigabit_ethernet}) 
% (\eg IEEE 802.3t standard \cite{ethernet_standard})
% and the link delays are randomly generated within $[25, 125]$ $\mu$s. Each switch has 2 hosts connected to it. 
We develop flow rules in the queues to enable connectivity among hosts in
different switches. The packets belonging to the real-time flows are queued
separately in individual queues and each of the queues are configured at a
maximum rate of $B_k \in [1, 5]$ Mbps. If the host exceeds the configured
maximum rate of $B_k$, our ingress policing throttles the traffic before it
enters the switch\footnote{In real
systems, the bandwidths allocation would be overprovisioned (as mentioned earlier), our evaluation takes a conservative approach.}. 

To measure the effectiveness of our prototype with mixed
(\eg real-time and non-critical) flows, we enable [1,3]
non-critical flows in the network.  All of the low-criticality
flows use a {\em separate, single queue} and are served in a FIFO manner -- it is the
``default'' queue in OVS. Since many commercial switches (\eg Pica8 P-3297, HPE FlexFabric 12900E, \etc) supports up to 8 queues, in our Mininet experiments we limit the maximum number of real-time flows to 7 (each uses a separate queue) and use the remaining 8th queue for non-critical flows. %Hence unless otherwise specified we set the number of flows $f_k = 7$.
Our flow rules isolate the
non-critical flows from real-time flows. All the experiments
are performed in an Intel Xeon 2.40 GHz CPU and Linux kernel version 3.13.0-100.

We use \texttt{netperf} (version 2.7.0)\cite{netperf} to generate the UDP traffic\footnote{Remember
that most hard real-time systems use UDP traffic \cite{rt_sdn_kaist, afdx_evolution}.} between the
source and destination for any flow $f_k$. Once the flow rules and queues are
configured, we triggered packets starting at the source $s_k$ destined to
host $t_k$ for each of the flows $f_k$. The packets are sent at a burst of 5
with 1 ms inter burst time. All packet flows are triggered simultaneously and
last for 10 seconds.

%For each set of flows $f_k \in \lbrace 2, 5 \rbrace$, 
  
%To observe the impact of delay budget in different network topology, we consider the end-to-end delay requirement $D_k,~ \forall f_k \in F$ as the function of topology. In particular, for each randomly generated network topology $G_i$ 
We assume flows are indexed based on priority, \ie $D_1 < D_2 < \cdots <
D_{|F|}$ and 
randomly generate 25
different network topologies. We set $D_1 = 100 \delta_i$ $\mu$s and increment with 10 for each of
the flow $f_k \in F, k>1$ where $\delta_i$ is the diameter of the graph $G_i$ in the $i$-th spatial
realization of the network topology. For each topology, we
randomly generate the traffic with required bandwidth $B_k \in [1, 5]$ Mbps and
send packets between source ($s_k$) and destination ($t_k$) hosts for 5 times
(each transmission lasts for 10 seconds) and log the worst-case round-trip
delay experienced by any flow. 



% \begin{figure}[!t]
% \centering
% \includegraphics[width=3.0in]{graphics/mhasan_delay_throughput}
% \caption{End-to-end round-trip delay and throughput with varying number of flows. For each set of flow $f_k \in \lbrace 2, 4, 7, 10, 12, 15, 20 \rbrace$, we examine $f_k \times 25 \times 5$ packet flows (each for 10 seconds) to obtain the experimental traces.}
% \label{fig:mhasan_delay_throughput}
% \end{figure}


%\paragraph{Experiment with synthetic network topology}

\subsubsection*{Experience and Evaluation}

\begin{figure}[t!]
\addtolength{\subfigcapskip}{-0.1in}
\centering
\subfigure[]{\includegraphics[width=\linewidth]{graphics/delay_mean_99p}
\label{fig:mhasan_mean_99p_delay}}%\hfil

% \subfigure[]{\includegraphics[width=3.3in]{graphics/delay_99p}
% \label{fig:mhasan_99p_delay}}%\hfil
\vspace*{-1.0em}
\subfigure[]{\includegraphics[width=\linewidth]{graphics/delay_max}\label{fig:mhasan_max_delay}}
%\hfil
%\hspace*{-1.9em}
\caption{(a) The empirical CDF of: (a) average and $99^{th}$ percentile, (b)  worst-case round-trip delay. %with different number of flows. For each set of flow $f_k \in \lbrace 2, 5 \rbrace$, we 
We set the number of flows $f_k = 7$ and
examine 7 $\times$ 25 $\times$ 5 packet flows (each for 10 seconds) to obtain the experimental traces.}
\label{fig:mhasan_delay}
\vspace{-0.2in}
\end{figure}

In Fig. \ref{fig:mhasan_delay} we observe the impact of number of flows on the
delay. Experimental results are illustrated for the schedulable flows (\viz the
set of flows for which \textit{both} delay and bandwidth constraints are
satisfied). 

The y-axis of Fig. \ref{fig:mhasan_delay} represents the empirical CDF of
average/$99^{th}$ percentile (Fig.
\ref{fig:mhasan_mean_99p_delay}) and worst-case (Fig. \ref{fig:mhasan_max_delay})
round-trip delay experienced by any flow. The empirical CDF is defined as
$G_\alpha(\jmath) = \frac{1}{\alpha} \sum_{i=1}^\alpha \mathbb{I}_{[\zeta_i
\leq \jmath]}$, where $\alpha$ is the total number of experimental
observations, ${\zeta}_i$ round-trip delay the $i$-th experimental observation,
and $\jmath$  represents the $x$-axis values (\viz round-trip delay) in Fig.
\ref{fig:mhasan_delay}. The indicator function $\mathbb{I}_{[\cdot]}$ outputs
1 if the condition $[\cdot]$ is satisfied and 0 otherwise. 

From our experiments we find that, the non-critical flows \textit{do not}
affect the delay experienced by the real-time flows and the average as well as the $99^{th}$
percentile delay experienced by the real-time flows \textit{always} meet their delay
requirements. This is because our flow rules and queue configurations isolate
the real-time flows from the non-critical traffic to ensure that the end-to-end
delay requirements are satisfied. We define the \textit{expected delay bound}
as the expected delay if the packets are routed through the diameter (\ie the
greatest distance between any pair of hosts) of the topology and given by
$\mathfrak{D}_i(u, v) \times  \delta_i$ and bounded by $[25 \delta_i, 125
\delta_i]$ where $\mathfrak{D}_i(u, v) \in [25, 125]$ is the delay between the
link $(u,v)$ in $i$-th network realization. As seen in Fig.
\ref{fig:mhasan_mean_99p_delay}, the average and
$99^{th}$ percentile round-trip delay are significantly less than the minimum
expected round-trip delay bound (\eg 2 $\times$ 25 $\times$ 4 = 200 $\mu$s).
This also validates the effectiveness of Algorithm
\ref{alg:mcp_path_delay_bw}. Besides, as seen in Fig.
\ref{fig:mhasan_delay}, the worst-case delay is also less than the maximum
expected delay bound (\eg 1000 $\mu$s) with probability 1. 


\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{graphics/boxplot_99p}\caption{End-to-end round-trip $99^{th}$ percentile delay with varying number of flows. For each set of flow $f_k \in [2, 7]$, we examine $f_k \times 25 \times 5$ packet flows (each for 10 seconds).% to obtain the experimental traces.
}
\label{fig:mhasan_delay_box}
\vspace{-0.1in}
\end{figure}

In Fig. \ref{fig:mhasan_delay_box} we illustrate the $99^{th}$ percentile round-trip
delay (represents the y-axis in the figure) with different number of flows
(x-axis). Recall that in our experimental setup we assume at most 8 queues are available in the switches where 7 real-time flows are assigned to each of 7 queues and the other queue is used for [1, 3] non-critical flows. As shown in Fig. \ref{fig:mhasan_delay_box}, increasing the number of flows slightly decreases quality of
experience (in terms of end-to-end delays). With increasing
number of packet flows the switches are simultaneously processing forwarding
rules received from the controller -- hence, it increases the round-trip delay. Recall
that the packets of a flow are sent in a bursty manner using \texttt{netperf}.
Increasing number of flows in the Mininet topology increases the packet loss and
thus causes higher delay. 

%As shown in Fig. \ref{fig:mhasan_max_delay}, with a small probability (\eg 0.25 and 0.35 when number of flows 2 and 5, respectively) we find the worst-case delay experienced by the flow is greater than the minimum round-trip delay budget (\eg 2 $\times$ 400 = 800 $\mu$s). Recall that the packets of a flow are sent at a burst using \texttt{netperf}. Increasing number of flows in Mininet topology increases the packet loss and thus causes higher worst-case delay. Again as we see from Fig. \ref{fig:mhasan_delay} the worst-case delay is also less than the maximum expected delay bound (\eg 1000 $\mu$s) and 
For our experiments with Mininet and \texttt{netperf} generated traffic, we do
\textit{not} observe any instance for which a set of schedulable flow misses its
deadline (\ie packets arriving {\em after} the passing of their end-to-end delay
requirements). Thus, based on our empirical results and the constraints provided to the path layout algorithm, we can assert that the schedulable real-time flows will meet their corresponding end-to-end delay requirements.

%Although the flows are schedulable (\eg delay and bandwidth constraints are satisfied), as we have illustrated in Fig. \ref{fig:mhasan_max_delay}, the worst-case delay experienced by the flows exceeds the expected delay bound with a probability greater than 0.6 especially for the large (\eg 8) number of flows. We attribute the fact  as an experimental artifact of Mininet. Increasing number of flows in Mininet topology increases the packet loss and thus causes higher worst-case delay. Our future work intends to explore the impact of worst-case delay with increasing number of flows in actual hardware switches.


==> For arxiv/experiment_param.tex <==
\begin{table}[!htb]
\vspace{-0.1in}
\renewcommand{\arraystretch}{1.2}
\caption{Experimental Platform and Parameters}
\label{tab:ex_param}
\centering
%\begin{tabular}{c||p{5.9cm}}
\begin{small}
\begin{tabular}{p{4.20cm}||p{3.30cm}}
\hline %\\
\bfseries Artifact/Parameter & \bfseries Values\\
\hline\hline
Number of switches & 5 \\
Bandwidth of links & 10 Mbps \\
Link delay & [25, 125] $\mu$s \\
%Number of real-time flows & $[2, 7]$ \\
Bandwidth requirement of a flow & [1, 5] Mbps \\
SDN controller & Ryu 4.7 \\
Switch configuration & Open vSwitch 2.3.0 \\
Network topology & Synthetic/Mininet 2.2.1 \\
OS & Debian, kernel 3.13.0-100\\
\hline
\end{tabular}
\end{small}
\vspace{-0.1in}
\end{table}


==> For arxiv/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We implement our prototype as an {\em application that uses the northbound API}
for the Ryu controller \cite{ryu}. The prototype application accepts the
specification of flows in the SDN. The flow specification contains the
classification, bandwidth requirement and delay budget of each individual flow. In order for a given flow $f_k$ to be realized in the network, the control-plane state of the SDN needs to be modified. The control-plane needs to route traffic along the path calculated for each $f_k$ as described in Section \ref{sec:algo}. In this section, we describe how this is accomplished by decomposing the network-wide state modifications into a set of smaller control actions (called Intents) that occur at each switch. 

% decomposition of a flow into smaller units that occur on switches
% makes it manageable
% 

%\begin{figure}[h!]
\begin{figure}%[h!]
\centering
\vspace*{-1em}
\includegraphics[width=2.75in]{graphics/intents_illustration.png}
\caption{Illustration of decomposition of a flow $f_k$ into a set of intents: $f_k$ here is a flow from the source host $h_1$ to the host $h_2$ carrying mission-critical DNP3 packets with destination TCP port set to $20,000$. In this example, each switch that $f_k$ traverses has exactly two ports.}
\label{fig:intents_illustration}
\vspace{-0.2in}
\end{figure} 

\subsection{Forwarding Intent Abstraction}

An \textit{intent} represents the {\em actions performed on a given packet at each
individual switch}. Each flow $f_k$ is decomposed into a set of intents as shown
in Figure \ref{fig:intents_illustration}. The number of intents that are
required to express actions that the network needs to perform (for packets in a
flow) is the same as the number of switches on the flow path. Each
intent is a tuple given by $(\mathsf{Match}, \mathsf{Input Port},
\mathsf{Output Port}, \mathsf{Rate})$. Here, $\mathsf{Match}$ defines the set
of packets that the intent applies to, $\mathsf{Input Port}$ and
$\mathsf{Output Port}$ are where the packet arrives and leaves the switch and
finally, the $\mathsf{Rate}$ is intended data rate for the packets matching the
intent. In our implemented mechanism for laying down flow paths, each intent
translates into a single OpenFlow \cite{specification20131} flow rule that is
installed on the corresponding switch in the flow path. 

\subsection{Bandwidth Allocation for Intents}
In order to guarantee bandwidth allocation for a given flow $f_k$, each one of
its intents (at each switch) in the path need to allocate the same amount of
bandwidth. As described above, each intent maps to a flow rule and the flow
rule can refer to a meter, queue or both. However, meters and queues are
precious resources and not all switch implementations provide both of them.
As mentioned earlier (Section \ref{sec:system_model}), 
% there exist two 
% alternative strategies for allocating bandwidth to individual intents:
% \ca individual queue/meter for each flow and
% \cb multiplexing meters and queues across multiple flows. The former strategy
% limits the rate of the queue/meter to $B_k$. It also places limits on the
% number of flows that a given switch can support at any point in time. On the
% other hand, as seen in Section \ref{sec:motivating_example}, it guarantees much 
% better isolation among flows. The second strategy (multiplexing) makes better
% use of the (limited) resources on each switch but cannot guarantee isolation
% without further changes to a switch's implementation. Hence, in our current
% implementation, 
we use the strategy of one queue per flow that guarantees 
better isolation among flows and results in stable delays.
%) and leave the multiplexing idea for future work.

\begin{comment}
\subsubsection{Individual Queue/Meter for the Flows}
This strategy uses one queue or one meter per flow. The service rate of the queue or the limiting rate of the meter is set to $B_k$. It limits the total number of flows that a given switch can support to the number of queues per port, or the total number of meters available at the switch. However, it guarantees full isolation among flows.

\subsubsection{Multiplexing Meters and Queues}
An alternative strategy for a switch implementing the optional traffic metering features, is to multiplex meters and queues available at a switch and generate appropriately sized slots for $B_k$ for each flow. For example, assume a queue set to be served at a rate 100 Mbps could \textit{fit} five flows with rates 20 Mbps. However, in order to guarantee full isolation among these flows now, each flow must also be metered at 20 Mbps, before its packets are enqueued. 

In our current implementation, however, we do not analyze the aforesaid multiplexing strategy and intend to explore the multiplexing issues in future work.
\end{comment}

\subsection{Intent Realization}
Each intent is realized by installing a corresponding flow rule by using the northbound API of the Ryu controller. Besides using the intent's $\mathsf{Match}$ and $\mathsf{Output Port}$, these flow rules refer to corresponding queue and/or meter. If the meters are used, then they are also synthesized by using the controller API. However, OpenFlow does not support installation of queues in its controller-switch communication protocol, hence the queues are installed separately by interfacing directly with the switches by using a switch API or command line interface. 


==> For arxiv/ingress_filtering.tex <==
Links to some useful articles:
\begin{enumerate}
\item IFB example\footnote{https://wiki.gentoo.org/wiki/Traffic\_shaping}
\item Ingress policing and IFB mirroring\footnote{ http://serverfault.com/questions/350023/tc-ingress-policing-and-ifb-mirroring}
\item Explanation redirection vs mirroring\footnote{http://fossies.org/linux/iproute2/doc/actions/mirred-usage}
\item HTB manual \& examples\footnote{http://luxik.cdi.cz/~devik/qos/htb/manual/userg.htm}
\item Classifying packets using tc filters\footnote{http://lartc.org/howto/lartc.qdisc.filters.html}
\item A video on tc classification system\footnote{https://www.youtube.com/watch?v\=cyeJYjZHv5M}
\end{enumerate}
Lessons learned -

==> For arxiv/intro.tex <==
\section{Introduction}
\label{sec:intro}
% \begin{itemize}
% \item Real-Time Systems vs Non-Real time system - network and QoS requirments. Need of hard real-time gurantees. Examples of different types of traffics and emphasizing on hard real-time traffic. (Basically setting the stage for problem formulation)
% \item Existing RT systems - examples - AFDX in avoinics, industrial networks
% \item Traditional computer networks - Diffserv/Intserv,  shortcomings 
% \item Leaverage SDN for real-time traffic with QoS 
% \item May cite few related work here. Details will be related work section.
% \item Aim of this paper, problem and approach outline, basic evaluation results summarization:  Three classes of traffic - Class 1 represents realtime flow with hard delay requirements (dead-lines).  Other two classes has soft delay requirments.  Goal is to build a framework that allows easy synthesis of network flows with the QoS requirements for three classes of traffic.  
      
% \item Paper organization
% \end{itemize}

% The networking requirements posed by real-time systems often require that tight bounds be met on maximum delay and bandwidth experienced by data flows. This in stark contrast to more conventional networking wherein packet delivery is often best-effort. 

% Traditionally, in order to connect components in a real-time system, specialized hardware and software has been used. [Some of the approaches to Real-time networking should get a passing mention here.]

% Software Defined Networking (SDN) is the insurgent networking architecture which advocated a centralized control-plane and thus allows tighter control on the behavior of individual networking elements. SDN has already been used to synthesize network flows that meet strict access control requirements, however it has not been used to provision QoS requirements as well.

% Thus, within the realm of SDN, the approach that we take is synthetic, i.e. we construct rules that provision the networking that a given real-time system requires. 

%\input{Analysis}
%1. Per switch delay: for each switch how much delay that it impose
%
%experiment: 1 flow with high priority with other flows on the network. Try to find out if this flow is affected by the other traffic. Check the worst case bound.
%2. Delay composition for per flow as well as 
%\cite{embeddedsecurity:mohan2014} 

% \todo[inline]{MH: title suggestions:

% SoRT: enabling \textbf{S}DN for	timing guarantees in hard \textbf{R}eal-\textbf{T}ime systems


% ** enabling/Towards end-to-end delay-awareness in SDN for real-time systems

% TIGRESS: Towards  \textbf{TI}ming Guarantees in Hard \textbf{RE}altime \textbf{S}ystems using \textbf{S}dn

% Towards  Timeliness/end-to-end Guarantees in real-time embedded systems using SDN

% GRoSS:	Towards timing \textbf{G}uarantee in hard \textbf{R}ealtime \textbf{S}ystems using \textbf{S}DN

% TwiSt:	 Towards Real-\textbf{T}me Guarantees in \textbf{S}oftware-Defined Networks

% RaTfiSh:	  Towards \textbf{R}eal-\textbf{T}ime Guarantees in \textbf{S}oftware-Defined Networks


% pRoGREsS: Towards \textbf{R}eal-Time \textbf{G}ua\textbf{R}ant\textbf{E}es in \textbf{S}oftware-Defined Networks}

Software-defined networking (SDN) \cite{mckeown2008openflow} has become increasingly popular since it
allows for better management of network resources, application of security
policies and testing of new algorithms and mechanisms. It finds use in a wide
variety of domains – from enterprise systems \cite{levin2013incremental} to cloud computing services \cite{jain2013network}, from
military networks \cite{spencer2016towards} to power systems \cite{pfeiffenberger2014evaluation} \cite{aydeger2016software}. The global view of the
network obtained by the use of SDN architectures provides significant advantages when compared
to traditional networks. It allows designers to push down rules to the various
nodes in the network that can, to a fine level of precision, manage the
bandwidth and resource allocation for flows through the entire network. However, current SDN architectures do not reason about delays. On the other hand, real-time systems (RTS), especially those with stringent timing constraints,
need to reason about delays. {\em Packets must be delivered between hosts with
guaranteed upper bounds on end-to-end delays}. Examples of such systems include
avionics, automobiles, industrial control systems, power substations,
manufacturing plants, \etc~ 

While RTS can include different types of traffic\footnote{For instance, 
\ca high priority/criticality traffic that is essential for the
correct and safe operation of the system; 
\cb medium criticality traffic that is critical to the correct operation
of the system, but with some tolerances in delays, packet drops, \etc; and 
\cc low priority traffic -- essentially all other traffic in the system 
that does not really need guarantees on delays or bandwidth such as engineering
traffic in power substations, multimedia flows in aircraft, \etc}, in this
paper we focus on the high priority flows that have stringent timing
requirements, predefined priority levels and can tolerate little to no loss of
packets.  We refer to such traffic as ``Class I'' traffic.  Typically, in many
safety-critical RTS, the properties of all Class I flows are well known, \ie
designers will make these available ahead of time. Any changes
(addition/removal of flows or modifications to the timing or bandwidth
requirements) will often require a serious system redesign. The number (and
properties) of other flows could be more dynamic -- consider the on-demand
video situation in an airplane where new flows could arise and old ones stop based on the
viewing patterns of passengers. 

Current safety-critical systems often have separate networks (hardware and
software) for each of the aforementioned types of flows (for safety and
sometimes security reasons).  This leads to significant overheads (equipment,
management, weight, \etc) and also potential for errors/faults and even
increased attack surface and vectors.  Existing systems, \eg avionics
full-duplex switched Ethernet (AFDX) \cite{ARINC2009,land2009,Charara2006},
controller area network (CAN) \cite{can2014}, \etc~that are in use in many of
these domains are either proprietary, complex, expensive and might even require
custom hardware. Despite the fact that AFDX switches ensure timing determinism,
packets transmitted on such switches may be changed frequently at run-time when
sharing resources (\eg bandwidth) among different networks
\cite{afdx_openflow}. In such situations, a dynamic configuration is required
to route packets based on switch workloads and flow delays to meet all the high
priority Quality of Service (QoS) requirements (\eg end-to-end delay). In
addition AFDX protocols require custom hardware \cite{afdx_evolution}.
% and may not easily be integrated with
% legacy RTS that uses commercial off-the-shelf (COTS) switches.

In this paper we present mechanisms to {\em guarantee end-to-end delays for
high-criticality flows (Class I) on networks constructed using SDN switches.}
The advantage of using SDN is that it provides a centralized mechanism for
developing and managing the system. The global view is useful in providing the
end-to-end guarantees that are required. Another advantage is that the
hardware/software resources needed to implement all of the above types of
traffic can be reduced since we can use the same network infrastructure
(instead of separate ones as is the case currently).  On the other hand, the
current standards used in traditional SDN (OpenFlow \cite{mckeown2008openflow,
specification20131}) generally do not support end-to-end delay guarantees or
even existing real-time networking protocols such as AFDX.  Retrofitting
OpenFlow into AFDX is not straightforward and is generally less effective
\cite{deterministic_openflow}.

A number of issues arise while developing a software-defined networking
infrastructure for use in real-time systems. For instance, Class I flows 
need to meet their \textit{timing} (\eg end-to-end delay) requirements
for the real-time system to function correctly. Hence, we
need to \textit{find a path} through the network, along with necessary resources, that will meet these
guarantees. However, current SDN implementations reason about resources like bandwidth instead of delays. Hence, we must find a way to extend the SDN infrastructure to reason about delays for use in RTS. Further, in contrast to traditional SDNs, it is not necessary to find the
\textit{shortest} path through the network. Oftentimes, Class I flows can
arrive \textit{just in time} \cite{Qian2015, Oh2015}, \ie just before their
deadline -- there is no real advantage in getting them to their destinations
well ahead of time. Thus, path layout for real-time SDN is a \textit{non-trivial}
problem since, \ci we need to understand the delay(s) caused by individual
nodes (\eg switches) on a Class I flow and \cii compose them along 
the delays/problems caused by the presence of other flows in
that node as well as the network in general.
%and \ciii generate backup
%paths to tolerate node/link failures. In this paper, we consider aspects
%\textit{i}) and \textit{ii}) and do not address the fault-tolerance issues.

In this work\footnote{A preliminarily version of the work is under submission to the 2017 RTN workshop that does not have published proceedings. In this paper we extend the workshop version with more comprehensive experiments (Section \ref{sec:evaluation}) and evaluation on actual hardware switches (Section \ref{sec:motivating_example}).} we consider Class I (\ie high-criticality) flows and develop a
scheme to meet their timing constraints\footnote{We will work on integrating
other types of traffic in future work.}. 
%However, the proposed mechanism can also
%be applied to the Class II traffic without loss of generality. 
We evaluate the effectiveness of the proposed approach with various custom
topology and UDP traffic (Section \ref{sec:evaluation}). The main contributions of this work are summarized as follows:

\begin{enumerate}
\item We developed mechanisms to guarantee timing constraints for traffic in hard real-time
	systems based on COTS SDN hardware (Sections
	\ref{sec:system_model}, \ref{sec:approach} and \ref{sec:algo}).

\item We illustrate the requirements for isolating flows into different queues
	to provide stable quality of experience in terms of end-to-end delays
	(Section \ref{sec:motivating_example}) even in the presence of other
	types of traffic in the system.
\end{enumerate}


%\hl{TODO: mention about workshop paper and highlight extensions. -- MH}

 %Perhaps, using this property, the path planning scheme can pack more flows into the system to use the network capacities more efficiently?



\begin{comment}
Another property of RTS is that they often
include traffic flows with mixed criticality, \ie those with varying degrees of
timing (and perhaps even bandwidth and availability) requirements: 
\ca {\em high priority/criticality traffic} that is essential for the
correct and safe operation of the system; examples could include sensors for closed loop control and
actual control commands in avionics, automotive or power grid systems; 
\cb {\em medium criticality traffic} that is critical to the correct operation
of the system, but with some tolerances in delays, packet drops, \etc; for instance,
navigation systems in aircraft, system monitoring traffic in power substations, \etc;
\cc {\em low priority traffic} -- essentially all other traffic in the system 
that does not really need guarantees on delays or bandwidth such as engineering traffic
in power substations, multimedia flows in aircraft, \etc~The high priority flows (that we henceforth refer to as ``Class I'' traffic)
have stringent timing requirements and can often tolerate little to no loss of
packets. Often these flows also have predefined {\em priority levels} among 
themselves.
\end{comment}

%If we take the example of an avionics system, then we could reasonably
%categorize the network flows within them into three classes:

\begin{comment}
\begin{enumerate}

\item \textit{Hard real-time/high-criticality traffic}:
In the avionics world, this could include the network flows that are used for the flight control, \ie I/O from engines, flaps, wind speed sensors, \etc ~-- essentially anything that is critical to the safe operation of the aircraft. Such traffic often has stringent timing requirements. There is also a need to guarantee that packet loss is minimized. The various flows could also have (predefined) priority levels among themselves. 

Let us refer to such flows as Class I traffic.

\item \textit{Soft real-time/medium-criticality traffic}: There are other applications that are critical to the correct operation of the aircraft. Their timing requirements, though tight and bounded, may not be as stringent as those in Class I. For instance, the navigation and mapping applications. Such flows can, potentially, tolerate a few missed packets from time to time. They could also include some laxity in their end-to-end delay requirements (\eg the packets meet their timing constraints with a 95\% confidence) but a more serious drop in the required guarantees could result in a serious degradation of the performance (and potentially safety) of the system. 

Let us refer to such network flows as Class II traffic.


As with Class I traffic, the flows can have priorities among themselves but it is well understood that all Class I flows have a higher priority than all flows in Class II.


\item \textit{Non (or very loose) real-time/low-criticality traffic}: This category is for capturing all other network flows in the system, say the internet traffic for customers, on-demand video playback, music streaming, \etc ~-- essentially anything else that is used for the routine operations in the system, including debug/engineering traffic. Some of these could have timing requirements (\eg video streaming) while other may not (\eg debug traffic). On the other hand the bandwidth requirements for this group of traffic could potentially be the highest. 

This can be labeled as Class III traffic.
\end{enumerate}
%\end{noindentlist}
\end{comment}



==> For arxiv/limitations.tex <==
\section{Discussion}
\label{subsec:limitations}

Despite the fact that we provide an initial approach to leverage the benefits of the SDN architecture to guarantee guarantee end-to-end delay in safety-critical hard RTS, our proposed scheme has some limitations and can be extended in several directions. To start with, %we intend to validate our implementations in actual hardware switches with more complex topology and analyze the worst-case latency experienced by the flows. Furthermore, 
most hardware switches limit the maximum number of individual queues\footnote{\eg Pica8 P-3297 and HPE FlexFabric 12900E switches support at most 8 queues.} that can be allocated to flows. Our current intent realization mechanism reserves one queue per port for each Class I flow. This leads to depletion of available queues. Hence, we need smarter methods to \textit{multiplex} Class I flows through limited resources and yet meet their timing requirements. Our future work will focus on developing sophisticated schemes for ingress/egress filtering at each RT-SDN-enabled switch. This will also help us better identify the properties of each flow (priority, class, delay, \etc) and then develop scheduling algorithms to meet their requirements. 

In this work we allocate separate queues for each flow and layout paths based on the ``delay-monotonic'' policy. However establishing and maintaining the flow priority is \textit{not} straightforward if the ingress policing requires to share queues and ports in the switches. Many existing mechanisms to enforce priority are available in software switches (\eg the hierarchical token buckets (HTB) in Linux networking stack). In our experience, enabling priority on hardware switches has proven difficult due to firmware bugs.

%Although we can satisfy the delay requirements for Class I and II flows by statically assigning priorities and careful path planning, this may cause starvation to the Class III flows and degrade overall network throughput (\eg bandwidth utilization). Therefore, one approach could be to dispatch the packets dynamically at each of the switches based on local decisions to provide better quality of experience (in terms of end-to-end delay and bandwidth utilization). For instance, if any flow at a given switch has stringent delay requirement (or starving due to higher-priority flows), it may locally assign higher priorities than the flows queued at that switch.  Therefore, that flow, even if queued/arrived later, may dispatch earlier to minimize the queueing delay at each of the hops (e.g., switches) in its route. Since the existing packet filtering mechanisms in Linux do not support this delay and priority-aware dynamic path routing policies, we need to develop of modify existing packet filtering mechanisms and verify the effectiveness analytically as well as through implementation/verification on hardware.

Finally, we do not impose any admission control policy for the unschedulable (\ie the flows for which the delay and bandwidth constraints are not satisfied) flows. One approach to enable admission control is to allow $m$ out of $k$ ($m < k$) packets of a low-priority flow to meet the delay budget by leveraging the concept of $(m,k)$ scheduling \cite{m_k_overload} in traditional RTS. 




==> For arxiv/mcp_base.tex <==
%\appendix

%\footnote{Line 3-17 in \textbf{Algorithm \ref{alg:mcp_org}} is similar to that of presented in earlier work \cite[Sec. 2.2]{mcp_klara} and for the purposes of this work, %we have extended the previous algorithm accordingly. we have extended this algorithm for our formulation.}

The heuristic solution of MCP problem, as summarized in Algorithm \ref{alg:mcp_org} works as follows. Let
\begin{equation}
%$$
\Delta(v,i) = \min\limits_{\mathcal{P} \in P(v,i)} W_1(\mathcal{P})
%$$ 
\end{equation}
where $P(v,i) = \lbrace \mathcal{P} ~|~ W_2(\mathcal{P}) = i, \mathcal{P} \text{ is any path from } s \text{ to } t \rbrace$ is the smallest $W_1(\mathcal{P})$ of those paths from $s$ to $v$ for which $W_2(\mathcal{P}) = C_2$. For each node $v \in V$ and each integer $i \in [0, \cdots, C_2]$ we maintain a variable $d[v, i]$ that keeps an estimation of the smallest $W_1(\mathcal{P})$. The variable initialized to $+ \infty$ (Line 3), which is always greater than or equal to $\delta(v,i)$. As the algorithm executes, it makes better estimation and eventually reaches $\Delta(v,i)$ (Line 8-15). %When the algorithm finishes the search for path (Line 17), $d[v, i] = \delta(v,i), \forall v \in V, \forall i \in [0, \cdots C_2]$. 
Line 3-17 in Algorithm \ref{alg:mcp_org} is similar to the single-cost path selection approach presented in earlier work \cite[Sec. 2.2]{mcp_klara} and for the purposes of this work, %we have extended the previous algorithm accordingly. 
we have extended the previous approach for our formulation.

We store the path in the variable $\pi[v,i], \forall v \in V, \forall i \in [0, \cdots, C_2]$. When the algorithm finishes the search for path (Line 17), there will  be a solution if and only if the following condition is satisfied \cite{mcp_klara} 
\begin{equation} \label{eq:path_cond}
%$
\exists i \in [0, \cdots, C_2],~~ d[t,i] \leq C_1.
%$ 
\end{equation}
If it is not possible to find any path (\eg the condition in Eq. (\ref{eq:path_cond}) is not satisfied), the algorithm returns False (Line 41). If there exists a solution (Line 19), we extract the path by backtracking (Line 21-29).
Notice that the variable $\pi[v, i]$ keeps the immediate preceding node of $v$ on the path (Line 13). Therefore, the path can be recovered by tracking $\pi$ starting from destination $t$ through all immediate nodes until reaching the source $s$. 
Based on this MCP abstraction, we developed a path selection scheme  considering delay and bandwidth constraints (Algorithm \ref{alg:mcp_path_delay_bw}) that works as follows.


\input{algorithm_mcp}

==> For arxiv/motivating_example.tex <==
\subsection{Queue Assignment Strategies}
\label{sec:motivating_example}

\begin{figure*}[htb]
\vspace{-1em}
\addtolength{\subfigcapskip}{-0.2in}
\centerline{\subfigure[]{\includegraphics[width=3in]{graphics/two_switch_topology_with_flows}
\label{fig:two_switch_topology_with_flows}}
\hfil
\hfill
\vspace*{-1em}
\subfigure[]{\includegraphics[width=3.5in]{graphics/delay_measurements_hardware.pdf}
\label{fig:delay_measurements}}\hfil}
\caption{Delay measurement experiments: (a) The two-switch, four host topology used in the experiments with the active flows. (b) The measured mean and $99^{th}$ percentile per-packet delay for the packets in the active flows in 30 iterations.}
\label{fig:motivating_example_figure}
\vspace{-0.2in}
\end{figure*}

We intend to synthesize configurations for Class I traffic such that it ensures
{\em complete isolation of packets for each designated class I flow}. 

In order to test how using output queues can provide isolation to flows
in a network so that each can meet its delay and bandwidth requirements
simultaneously, we performed experiments using OpenFlow enabled hardware switches\footnote{We also conduct similar experiments with software simulations (\eg by using Mininet \cite{lantz2010network} topology) and observe similar trends (see Appendix \ref{appsec:mininet_simple_topo}).}. The experiments use a simple topology that contains two white box Pica8 P-3297 \cite{pica8} switches (\texttt{s1},
\texttt{s2}) connected via a single link as shown in Figure
\ref{fig:motivating_example_figure}(a). Each switch has two hosts connected to
it. Each host is a Raspberry Pi 3 Model B \cite{raspberry} running Raspbian Linux. 

We configured flow rules and queues in the switches to enable connectivity
among hosts at one switch with the hosts at other switch. We experimented with
two ways to queue the packets as they cross the switch-to-switch link:
\ci in one case, we queue packets belonging to the two flows {\em separately} in two queues
(\ie each flow gets its own queue), each configured at a maximum rate of 50 Mbps
\cii in the second case, we queue packets from both flows in the {\em same queue}
configured at a maximum rate of 100 Mbps. 

After configuring the flow rules and queues, we used 
\texttt{netperf} \cite{netperf} to generate following packet flows: the first starting at the host \texttt{h1s1} destined to
host \texttt{h1s2} and the second starting at host \texttt{h2s1} with a destination 
host \texttt{h2s2}. Both flows are identical and are triggered simultaneously to last for 
15 seconds. We changed the rate at which the traffic is sent across both flows to measure the average per-packet delay. Figure \ref{fig:motivating_example_figure}(b) plots the average value
and standard error over 30 iterations. The x-axis indicates the rate at which
the traffic is sent via \texttt{netperf}, while the y-axis shows the average per-packet delay. The following key observations stand out:
\begin{enumerate}
	\item  The per-packet average delay increases in both cases
	as traffic send rate approaches the configured rate of 50 Mbps. This is
	an expected queue-theoretic outcome and motivates the need for slack
	allocations for all applications in general. For example, if an
	application requires a bandwidth guarantee of 1 Mbps, it should be
	allocated 1.1 Mbps for minimizing jitter.
\item The case with separate queues experiences lower average per-packet delay when flow rates approach the
	maximum rates. This indicates that when more than one flow
	uses the same queue, there is interference caused by both flows to
	each other. This becomes a source of unpredictability and eventually may
	cause the end-to-end delay guarantees for the flows to be not met or perturbed
	significantly.
\end{enumerate}

Thus, {\em isolating flows using separate queues results in lower and more stable
delays} especially when traffic rate in the flow approaches the configured maximum rates.
The maximum delay along a single link can be measured. Such measurements can
then be used as input to a path allocation algorithm that we describe in the following section.



==> For arxiv/problem_overview.tex <==
\section{Problem and System Overview}
\begin{itemize}
\item Three classes of traffic
\item Qos requirements - Bandwidth and Delay
\item Focuses on Class 1
\item Problem Statement
\item The big picture as what we are trying to do - Framework (figure) overview with different components and the communication flow among them.\\
- Network Manager - Maintains/obtains details statistics of the networks from the controller\\
- Path Allocation Algorithms with QoS - Routing/Paths layout.\\        ------ Theoretical model to obtain upper bound on end-to-end delay. 
   
- Admission Control
\item Evaluation with network emulator with OVS and real-switches

\end{itemize}

==> For arxiv/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%\todo[inline]{
%1. related works on CAN

%2. FlexRay?

%3. Cones %\url{http://energy.gov/sites/prod/files/CEDS%202010%20Peer%20Review%20-%20Converged%20Networks%20for%20SCADA%20-%20Himanshu%20Khurana,%20Illinois.pdf}
%}

There have been several efforts to study the provisioning a network such that
it meets bandwidth and/or delay constraints for the traffic flows. Results from
the network calculus (NC) \cite{le2001network} framework offer a concrete way
to model the various abstract entities and their properties in a computer
network. NC-based models, on the other hand, do not prescribe any formulation
of flows that meet given delay and bandwidth guarantees. For synthesis, the
NP-complete MCP comes close and Shingang \etal formulated a heuristic algorithm
\cite{mcp_klara} for solving MCP. We model our delay and bandwidth constraints
based on their approach. 

% In traditional networks, provisioning for real-time applications is hampered by
% a distributed control-plane. The routers function as a distributed system and
% \textit{eventually} reach consensus about that a given application's packets.
% This consensus requires special protocols such as RSVP \cite{zhang1993rsvp}.
% Given that added layer of complexity, Integrated Services \texttt{IntServ}
% \cite{clark1992supporting} architecture was proposed in the mid 1990s for
% provisioning networks for real-time applications. Our approach of explicit
% resource allocation based on requirements of the application lines up with the
% principles behind \texttt{IntServ}. Finally,recent 
There are recent standardization efforts
such as IEEE 802.11Qbv \cite{ieee80211qbv} which aim to codify best practices for provisioning QoS using Ethernet. These approaches focus entirely on meeting guarantees and do not attempt to optimize link bandwidth.  However, the global view of the network provided by the SDN architecture allows us to optimize path layouts by formulating it as an MCP problem.

%With the rise of SDN architecture, 
There have been some prior attempts at provisioning SDN with worst-case delay
and bandwidth guarantees.  Azodolmolky \etal proposed a NC-based model
\cite{azodolmolky2013analytical} for a single SDN switch that provides an upper
bound on delays experienced by packets as they cross through the switch. Guck
\etal used mixed integer program (MIP) based formulation
\cite{guck2014achieving} for provisioning end-to-end flows with delay
guarantees -- they do not provide a solution of what traffic arrival rate to
allocate for queues on individual switches for a given end-to-end flow. 

A QoS-enabled management framework to allow end-to-end communication over SDN is proposed in literature \cite{Xu2015}. 
%It classifies flows into two levels, \ie QoS flow and best-effort. 
It uses flow priority and queue mechanism to obtain QoS control to satisfy the requirement  but did not demonstrate schedulability under different constraints.  A scalable routing scheme was developed in literature \cite{rt_sdn_kaist} that re-configures existing paths and calculates new paths based on the global view and bandwidth guarantees. The authors also present a priority ordering scheme to avoid contention among flows sharing the same switch. However, the basic requirement of the model used in that work (\ie end-to-end delay being less than or equal to minimum separation times between two consecutive messages) limits applicability of their scheme for a wide
range of applications. 

%They did not take into account hard real-time delay \hl{constraints.}    
Avionics full-duplex switched Ethernet
(AFDX)~\cite{ARINC2009,land2009,Charara2006} is a deterministic data network
developed by Airbus for safety critical applications. %based on COTS components
%and is being used in aircraft such as Airbus A380. 
The switches in AFDX architecture are interconnected using full duplex links, and static paths with
predefined flows that pass through network are set up. 
%For setting up a
%connection, a logical connection known as virtual link (VL) is set up over the
%network from source to end system with parameters bandwidth allocation gap
%(BAG) and minimum and maximum VL frame lengths. 
Though such solutions aim to
provide deterministic QoS guarantees through static routing, reservation and isolation, they
impose several limitations on optimizing the path layouts and on different
traffic flows. 
There have been studies towards evaluating the upper bound on the end-to-end
delays in AFDX networks\cite{Charara2006}. The evaluation seems to depend on the AFDX
parameters though.

% Several studies investigated the delay introduced by a scheduling algorithm implemented in the
% switch to route the packets through the switching fabric
% \cite{gopalakrishnanswitch,kang2013design,wang2010adapting}. 
% %The earlier work
% %indicates that deriving processing delays is not trivial for certain common
% %scheduling algorithms such as iSLIP \cite{McKeown:1999:ISA:310888.310896}. 
% %Hence, alternative algorithms that are more amenable to bounding the
% %delay were proposed. 
% Delay bounds in switching devices can not provide
% real-time guarantees for the whole network per se, but they must be considered
% when designing such network. The authors \cite{gopalakrishnanswitch} build
% on this knowledge and propose an algorithm
% to construct close-to-optimal network of switches that meets real-time
% requirements. Our approach is different in a sense that we consider existing
% network topology that can be arbitrarily complex.

There are several protocols proposed in automotive communication networks
such as controller area network (CAN) \cite{can2014} and FlexRay \cite{flex2016}. 
%CAN~\cite{can2014} is the
%international standard for in-vehicle communication in the automotive industry.
%It is peer-to-peer network and transmit a CAN frame when the bus is not busy
%and if multiple nodes try to transmit, the node with highest priority get the
%access. FlexRay~\cite{flex2016} uses TDMA scheme to  manage multiple nodes and
%allows complex network topology.
These protocols are designed to provide strong real-time guarantees but have limitations in how to extend it to varied network lengths, different traffic flows and complex network topologies. With SDN architectures and a flexible QoS framework 
proposed in this paper, one could easily configure COTS components and
meet QoS guarantees with optimized path layouts. % and backup paths.

Heine \etal proposed a design and built a real-time middleware system, CONES
(COnverged NEtworks for SCADA) \cite{Heine2011} %, known as CONES: COnverged NEtworks for SCADA, 
that enables the communication of data/information in SCADA
applications over single physical integrated networks. 
%To provide end-to-end
%real-time guarantees for SCADA applications over such integrated networks,
%host-based process management, network and host-based resource management
%solutions were integrated into the system. 
% These solutions leveraged some of
% the existing IP technologies such as Multiprotocol Label Switching (MPLS) and DiffServ for network resource reservation/management, and uses %iDSRT\cite{Nguyen2009} that uses 
% Earliest deadline first scheduling algorithm (EDF)
% for scheduling of network traffic and CPU time based on the deadline
% requirements.
However, the authors did not explore the synthesis of
rules or path optimizations based on bandwidth-delay requirements -- all of which are carried out by our system.
%. Taking
%advantages of SDN architecture, our framework supports synthesis of rules,
%paths set up and optimization based on delay-bandwidth requirements so that
%maximum number of flows can meet their guarantees. 
Qian \etal implemented a hybrid EDF packet scheduler \cite{Qian2015} for
real-time distributed systems. The authors proposed a proportional bandwidth sharing strategy based on number
of tasks on a node and duration of these task, due to partial information of the network.
% The scheduler transmits messages with a delay
% introduced by periodic message receiving task that accepts messages from the
% network buffer and releases to the EDF scheduler queue. This approach makes the
% system more predictable. At the network level, to reduce network delay variance,
% the scheduler is integrated with Linux traffic control and is used in
% combination with hierarchical token bucket (HTB). The network interface with
% HTB is configured for two queues (\viz real-time and background traffic) and
% priorities. %This approach required prior information on IPs and ports. 
% The authors proposed a proportional bandwidth sharing strategy based on number
% of tasks on a node and duration of these task. Though these strategies were
% adopted to make the system more predictable, due to partial information of
% the network, it leaves lots of scope for improvements.
In contrast, the SDN
controller has a global view of the network, thus allowing for more flexibility to
synthesize and layouts the paths and more control on the traffic.  

The problem of end-to-end delay bounding in RTS is addressed in literature~\cite{Jin2013}. The authors choose avionics systems composed of end devices,
%such as cameras and intermediate switching devices as a motivating example
and perform timing analysis of the delays introduced by end points and the
switches. However, the proposed approach requires modification to the
switches. Besides the authors do not consider the bandwidth limitations,
variable number of flows and flow classifications. 
%(real-time vs non-real-time).

There is a lot of work in the field of traditional real-time networking (too many
to enumerate here) but the focus on SDN is what differentiates our work.



==> For arxiv/simple_topo_mininet.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=3.5in]{graphics/delay_measurements.pdf}
\caption{The mean and $99^{th}$ percentile per-packet delay for the packets in the active flows in 25 iterations using a two-host four-switch (see Fig. \ref{fig:delay_measurements}) Mininet topology.}
\label{fig:mininet_delay_measurements}
\end{figure}
We also perform experiments with a two switch, four host topology similar that of presented in Section \ref{sec:motivating_example} using Mininet. The purpose of this experiment is to observe the performance impact on software simulations (\eg Mininet topologies) over the actual ones  (hardware switches and ARM hosts).
As we can see in Fig. \ref{fig:mininet_delay_measurements} the trends (\eg isolating flows using separate queues results in lower
delays) are similar in both Mininet and hardware experiments -- albeit the latencies are higher due to it being a software simulation and also affected by other artifacts (\eg the experiments are involved in generating traffic on the same machine).





==> For arxiv/skm_API.tex <==
\section{Secure Kernel Module API}\label{sec:skm_API}

==> For arxiv/system_model.tex <==
\section{System Model}
\label{sec:system_model}

Consider an SDN topology ($N$) with open flow switches and controller and a set
hrof real-time flows ($F$) with specified delay and bandwidth guarantee
requirements. The {\em problem is to find paths for the flows (through the 
topology) such that the flow requirements (\ie end-to-end delays) 
can be guaranteed for the maximum number of critical flows}.
We model the network as an undirected graph $N(V,E)$ where $V$ is
the set of nodes, each representing a switch port in a given network and $E$ is
set of the edges\footnote{We use the terms \textit{edge} and \textit{link}
interchangeably throughput the paper.}, each representing a possible path for
packets to go from one switch port to another.  Each port $v \in V$ has a set
of queues $v_q$ associated with it, where each queue is assigned a fraction of
bandwidth on the edge connected to that port.  

Consider a set $F$ of unidirectional, real-time flows that require delay and bandwidth
guarantees. The flow $f_k \in F$ is given by a four-tuple $(s_k, t_k,
D_k, B_k)$, where $s_k \in V$ and $t_k \in V$ are ports (the source 
and destination respectively) in the graph, $D_k$ is
the maximum delay that the flow can tolerate and $B_k$ is the maximum required
bandwidth by the flow. We assume that flow priorities are distinct and the
flows are prioritized based on a \textit{``delay-monotonic''} scheme \viz
the end-to-end delay budget represents higher priority (\ie $pri(f_i) > pri(f_j)$ if
$D_i < D_j,~ \forall f_i, f_j \in F$ where $pri(f_k)$ represents priority of
$f_k$). 
%\todo[inline]{Note that the delay experienced by a flow over a path could be due to processing time of a packet at a switch, propagation on physical link, transmission, and queuing at the ingress/egress port of a switch.}

For a flow to go from the source port $s_k$ to a destination port $t_k$, it
needs to traverse a sequence of edges, \ie a flow path $\mathcal{P}_k$. The
problem then, is to synthesize flow rules that use queues at each edge $(u,v) \in
\mathcal{P}_k$ that can handle \textit{all} flows $F$ in the given system
while still meeting each flow's requirement. If $d_{f_k}(u,v)$ and $b_{f_k}(u,v)$ is
the delay faced by the flow and bandwidth assigned to the flow at each edge
$(u,v) \in E$ respectively, then $\forall f_k \in F$ and $\forall (u,v) \in
\mathcal{P}_k$ the following constraints need to be satisfied:

\begin{align}%\label{eqn:constraints}
\sum_{(u,v)\in \mathcal{P}_k} d_{f_k}(u,v) &\leq D_k, \quad \forall f_k \in F  \label{eq:con_delay}\\
b_{f_k}(u,v) &\geq B_k, \quad \forall (u,v) \in \mathcal{P}_k, \forall f_k \in F. \label{eq:con_bw}
\end{align}

This problem needs to be solved at two levels:
\begin{itemize}
\item \textit{Level 1}: Finding the path layout for each flow such that it
	satisfies the flows' delay and bandwidth constraints. We formulate this
	problem as a multi-constrained path (MCP) problem and describe the
	solution in Sections \ref{sec:approach} and \ref{sec:algo}.
\item \textit{Level 2}: Mapping the path layouts from Level 1 on to the
	network topology by using the mechanisms available in OpenFlow. We
	describe details of our approach in Section~\ref{sec:implementation}.
\end{itemize}
%\todo[inline]{RBB-- not sure the two steps below are independent. Only independent if we assume individual queues}

%\todo[inline]{Rewritten -- does that less ambiguous? -- MH}
%Once we obtain path layouts that can satisfy the constraints specified by Eq.~\ref{eqn:constraints}, 

In addition to the aforementioned delay and bandwidth constraints (see Eqs.~(\ref{eq:con_delay}) and (\ref{eq:con_bw})), we need to map flows assigned to a port to the queues at the port. Two possible
approaches are: 
\ca {\em allocate each flow to an individual queue} or 
\cb {\em multiplex flows onto a smaller set of queues} and dispatch the packets based on priority. In fact, as we illustrate in the following section, the queuing approach used will impact the delays faced by the flows at each link. Our intuition is that
the {\em end-to-end delays are lower and more stable} when {\em separate queues}
are provided to each critical flow -- especially as the rates for the flows
get closer to their maximum assigned rates. Given the deterministic nature of many RTS, the number of critical flows are often limited and well defined (\eg known at design time). Hence, such over-provisioning is an acceptable design choice -- from computing power to network resources (for instance one queue per critical real time flow). We carried out some experiments 
to demonstrate this (and to highlight the differences between these two strategies) 
-- this is outlined in the following section. 

%As we discussed in the
%Section~\ref{sec:motivating_example}, the end-to-end delay is lower and more
%stable when separate queues for flows are used and rate of flow reaches maximum
%configured rate. Therefore, in this work we consider to use separate queues for
%each flow at each port. 



%Let $F_e$ \hl{@smruiti, @ rakesh k. : why not $F$? are we referring some different set of flows by $F_e$? -- mnwr.hsn} and $F_{eq}$ denotes the set of flows assigned to a port \textit{to be} mapped to queues and set of flows assigned to a queue $q$ at a port $e$. Lets assume we are given priority ($pri_k$) of each flow $f_k$, bandwidth allocated to each flow at port $e$, and the bandwidth assigned to each queue ($b_{eq}$).
% \begin{equation}
% b_{eq} \ge \sum_{f \in F_{eq}}b_{fe} 
% \end{equation}

%Then the above equation reduces to: $\forall f_k \in F_e$ and $k = 1 \cdots |F_e|$
% \begin{equation}
% b{eq}_k \geq B_k
% \end{equation}
% \todo{is this equation okay?}

%Depending on how we distribute the flows among queues based on flow priorities or based on priorities of each queue.

%Distribute hard real time flows to different queues. Need to find good mix of flows for each queue.

% There are three sources of packet delays: delay caused by processing of a packet at a switch, delay caused by propagation of packets among switches, and delay caused by queuing of packets at one or more ports at  in the network. If on each port, more bandwidth than the required bandwidth $B_k$ for the flow is reserved for the flow, then the flow experiences no queuing delays in the network. 



==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

LATEX = pdflatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> design.tex <==
\section{Design}
\label{sec:design}

% We consider following broad classes of requirements:

% Class 1: perflow, hard real time guarantee, control applications in avionics (AFDX)

% class 2: Fairness and soft real time, avionics infrastructure,  autopilot few miliseconds delay, (papers?)
% class 3: entertainment systems, (everything else)

There are three elements of the QoS Synethsis that we tackle separately:

1. Admission Control (Book-keeping, incremental addition of flows as system evolves)

2. Intent Generation (Graph Theory Aborescenes): 

3. QoS Paramater for Intents (Which queue a given intent uses at a switch, what the rate of the queue is set to, what queueing discipline is applied)



We take as input the set of flows that require to be synthesized.

We then compute the following:

1. The ingress filtering rules keep applications honest and limit them at the ingress.

2. We compute rules at each individual switch that need to be installed in order for all the required flows to meet the guarantees.

3. We compute parameters such as traffic rates and the queuing discipline used by packet queues that are referred by the flow rules computed previously.

Each one of these is accomplished as following:

\subsection{Ingress Filtering}
\input{ingress_filtering}
\subsection{Rules Computation}
\subsection{Packet Queue Parameter Computation}




==> detailed_arch.tex <==
\section{Detailed Architecture}
\label{sec::detailed_arch}

We now present more details about our \SKM{}-based two-level monitoring
architecture. The overall process is presented in Figure 
\ref{fig::overall_process}. We first explain this high level flow
and then delve into the details in the following sections.

\subsection{\SKM{} Architecture Operations}
\label{subsec::skm_operations}

Consider the example of detecting problems in the system call table (presented
in Section \ref{subsec::example_use_cases}). To understand the sequence of operations in our system, we describe in detail each step shown in Figure~\ref{fig::overall_process}:
\begin{enumerate}
	\item The \SKMMan{} sends the command to check the system call table. This
		command is written in the secure memory that is part of the \SKMHW{}.
	\item The above process results in an inter-core interrupt that is handled
		by an interrupt handler on the monitored core.\footnote{We will use
		`monitored core', `application core' and `main core' interchangeable.}
		We implement an interrupt-service routine to handle this specific
		interrupt, {\tt skm\_ISR()}.
	\item The ISR calls into the \SKM{} ({\tt skm\_tasklet()}) that handles
		the command sent by the \SKMMan{}. The \SKM{} then determines what
		exact command was called (in this case it was instructed to copy
		the system call table). No entity on the main core (other than the 
		\SKM{}) can decipher the command because access to the secure memory 
		is restricted. 
	\item The tasklet calls the appropriate function to carry out the required task
		\ie gather the information requested by the \SKMMan{}.
	\item The function (e.g., to copy the system call table) carries out its
		operations by placing the required information in the secure
		memory of the \SKMHW{}. 
	\item The secure core receives an interrupt that the data it requested is
		now available in the secure memory. On receiving the interrupt, 
		the \SKMMan{} starts to read out the information from the secure memory 
		region and then sends it to the appropriate module in the secure 
		core that can analyze this information.
\end{enumerate}
The above process repeats for every command that is sent by the \SKMMan{} to the \SKM{}.
Let us now look at more of the details that enable the above process.


\subsection{\SKM{} Setup}
\label{subsec::skm_setup}

The \SKM{} is loaded onto the monitored core during the OS booting phase. As mentioned in the threat model, we make the assumption here that the system is in a clean state at boot time. For this, one can use a secure-boot mechanism such as IMA~\cite{sailer2004design}. 

\begin{figure}[tb]
   \centering
   \includegraphics[width=0.95\columnwidth]{Figures/registration.pdf}
   \caption{\SKM{} registration during secure boot}
   \label{fig::registration}
\end{figure}

The first task for the \SKM{} (during load time) is to request the \SKMMan{} to 
register it, \ie authenticate itself (Figure \ref{fig::registration}). 
For the \SKMMan{} to test the veracity of
the \SKM{} request for registration, it uses a hash of the \SKM{}'s {\tt .text} section.
The \SKMMan{} then compares this newly computed hash with the value that was
obtained at design time (and is stored in the secure core). We do not trust
the \SKM{} yet---hence, we do not wait for the \SKM{} to send its hash but rather
calculate it independently in the \SKMMan{}. This prevents the situation where
a malicious module could copy the \SKM{}'s hash and try to pass off as the
legitimate module.

The \SKMMan{} needs the following information about the \SKM{} to compute this
hash value: \ca the virtual base address, \cb the size of the {\tt .text}
section, \cc the page size and the \cd page table information---all for the
\SKM{}. In ARM processors, the last piece of information corresponds to the translation
table base register 0 ({\tt TTBR0}) that holds the physical address of the
first level translation table $0$.\footnote{Depending on the OS and the
system configuration, the translation table base register $1$ ({\tt TTBR1})
may also be required in addition to {\tt TTBR0}. In our implementation the
\SKMMan{} is provided with both {\tt TTBR0} and {\tt TTBR1}, which
does not change the authentication process} The \SKMMan{} then translates the 
{\tt .text} section of the \SKM{} as defined by the base (virtual) address and 
its size to a set of physical addresses that host the \SKM{} code.

As shown in Figure \ref{fig::registration}, the \SKMMan{} then calculates a
hash of the data stored in the pages that store the \SKM{} code using 
the \textsf{SHA-1} algorithm. If the newly computed hash matches
what was calculated before (\ie at the time the \SKM{} was developed) then
the \SKMMan{} registers the base address for the \SKM{}'s {\tt .text} section, 
its size and {\tt TTBR0} with the \SKMHW{}. From then on, the secure memory
in the \SKMHW{} can only be access by the monitored core when it is executing
code that is known to be part of the \SKM{}.

%\todo[inline]{The following paragraph somehow does not make sense
%to me -- Sibin.}
%\note If the physical addresses of the \SKM{} were provided to the \SKMMan{} during
%the registration process, then a malicious module can claim itself to be
%the \SKM{} by mapping its own virtual address information to the \SKM{}'s
%physical addresses. Thus, the malicious module would pass the authentication
%because the original \SKM{}'s hash will be used. It could then access the secure 
%memory since its virtual address is registered with the \SKMHW{}. Our approach 
%of transferring the responsibility of translating the virtual to physical 
%address mapping to the \SKMMan{} prevents such attacks because the addresses
%used for the authentication as well as checking the access to the secure
%memory are the same.


\subsection{Secure Memory and Access Control}
\label{subsec::secure_memory}

\begin{figure}[t] 
\centering
\includegraphics[width=1\columnwidth]{Figures/secure_memory.pdf}
\caption{Secure memory access control on the \SKMHW{}.}
\label{fig::secure_memory}
\end{figure}

The secure memory on the on-chip \SKMHW{} unit is a key component in our
architecture. This memory enables secure and trusted communication between the
\SKM{} and the \SKMMan{}. A `secure memory controller' (associated with the
\SKMHW{}) only allows instructions that are part of the \SKM{} to access this on-chip
memory, at least from the main core.\footnote{Of course, any process on the
secure core can access this secure memory---this is guaranteed by
checking if the access requests are coming from the secure core.} To
implement this type of `access control', we need to check {\em who is
executing} on the monitored core when a memory transaction is issued
for the secure memory. The \SKMHW{} accesses the program counter register
({\tt PC}) on the main core (a virtual address) as well as the {\tt
TTBR0} register. It then checks if
\ci the {\tt TTBR0} register matches the one registered by the \SKM{} (as 
explained in Section \ref{subsec::skm_setup}) and
\cii the value of the {\tt PC} register is within the {\tt .text} region
of the \SKM{}. This ensures that only \SKM{} can access the secure on-chip memory. If the memory
controller detects an illegal access attempt (\ie access by a process
different from the \SKM{} or instructions that lie outside its legitimate
range) then the \SKMHW{} raises an alert and notifies the \SKMMan{}. The latter
can then take appropriate actions to counter the problem. Figure 
\ref{fig::secure_memory} presents this process.
 
However, it is entirely likely that a smart adversary may have modified the
address mapping thus making it look like its own instructions that falls
within the allowed virtual address space now points to different physical
addresses (that actually hosts malicious code instead of the \SKM{}). Hence,
the above access control mechanism will fail to prevent the malicious code
from access the secure memory. To prevent such issues, we could check the
physical addresses of the instructions trying to access the on-chip memory
to see if it falls within the expected range (of the \SKM{}). However,
we avoid this option since it would involve an address translation each time
the secure memory is accessed---this would result in huge performance
overheads. Our solution (as will be elaborated in Section \ref{subsec::heartbeat})
is for the \SKMMan{} to \ca translate the \SKM{}'s {\tt .text}
section from virtual to physical addresses and \cb calculate the hash of the
resultant pages---following exactly the same process as the registration, only
done often during execution, not just at boot time.
As long as the resultant hash value matches the original we can be sure that
the \SKM{} has not been tampered with.\footnote{Of course, this does not eliminate
the possibility where a carefully constructed malicious module changes the
address mappings and restores it to the original between two hash check points.
However, regular hashing with random time intervals can significantly reduce
the possibility of success for such attempts.}

Because of this stringent access control for the secure memory, we 
may not be able to use some kernel library functions, \eg \textsf{printk}. This is
particularly true if the arguments for such library functions (a string
in this case) is stored in the secure memory since the program counter
for the library function will fall outside the acceptable range of the
\SKM{}'s {\tt .text} region. One way to get around this issue is to write a 
wrapper function in the \SKM{} that copies the required data to some part of
the main memory and then pass it to the required library functions. 
There will never be an instance when sensitive data is passed outside
of the \SKM{} (or the \SKMHW{} memory module).

\subsection{Heartbeat and \SKM{} Integrity Check}
\label{subsec::heartbeat}

As mentioned earlier, we need to periodically check if 
\ci the \SKM{}'s code has not been tampered with;
\cii the \SKM{} is actually starting up when it is commanded to do so by the \SKMMan{}
and finally, \ciii the \SKM{} responds to requests in a timely manner.
We have already discussed a technique to check for \ci -- periodically
hash the {\tt .text} region of the \SKM{} and check against previously stored
values. The issues of liveness of the \SKM{}, \viz~\cii and \ciii, require a
more active approach on behalf of the \SKMMan{}.

Our solution for this problem is to send out a special command, every once
in a while, to the \SKM{}. The \SKM{} should respond to this command right away.
This ensures that the \SKM{} has not be deactivated by an adversary. No other
process/code can respond to this command since the communication happens 
through the secure memory that has a form of access control implemented
on it (Section \ref{subsec::secure_memory}). When the special command is
sent to the \SKM{}, the \SKMMan{} starts a countdown timer ($500 ms$ in our experiments). If it 
does not receive the expected response from the \SKM{} then this is also 
indicative of an attack. The timer can be used for any/all commands that
the \SKMMan{} sends across -- if the responses/information does not start
arriving before the timer expires then the \SKMMan{} can raise an alert and
assume that the \SKM{} has been attacked.

Another precaution that we can take is to send out these heartbeat commands at {\em random} intervals so that an adversary 
cannot guess the pattern of checks by the \SKMMan{}.


\subsection{Inter-core Interrupts for Communication}
\label{subsec::interrupts}

As mentioned earlier, we use inter-core interrupts to initiate communications
between the main and secure cores. When the \SKMMan{} sends a command via the
secure memory, it results in an interrupt to the monitored core. This interrupt
is handled by the \SKM{}'s interrupt service routine. For the sake of efficiency,
we use the `tasklet' mechanism in Linux. The code in the tasklet
parses the command from the \SKMMan{}. It calls whatever functions that are
required (and part of the \SKM{}) to complete the task. The results of the operation(s)
are placed back into the secure memory region. This generates another inter-core
interrupt but this time on the secure core side. The \SKMMan{} handles this interrupt
and routes the information to the appropriate analysis module.

The tasklet on the \SKM{} is not synced with the interrupt service routines. There
is a small chance that some finite time passes between the ISR invoking the
tasklet and the latter being scheduled to run. Hence, an attacker may prevent
the tasklet from executing. Hence, as mentioned in Section
\ref{subsec::heartbeat} the \SKMMan{} uses a timeout mechanism. When a command is
sent, a countdown timer is started. The expiration of the time (before
receiving any results from the other side) is a strong indicator of the main
core (and the \SKM{} in particular) being under attack.

When an interrupt is raised and handled by the \SKM{}, the first
step taken by an ISR is to change the stack pointer (for a context switch). This
could result in problems if the main stack is attacked by the adversary. Hence, 
we allocate the stack for the \SKM{} in the secure on-chip memory. We change the
stack pointer every time (to a random part of the secure memory) the \SKM{} 
handles an interrupt.

Since we will place the ISR in the \SKM{}'s {\tt .text} section, any attempts by
the attacker to change the ISR will be detected by the mechanisms mentioned earlier.
If, on the other hand, the main core's interrupts are disabled (especially the
inter-core interrupts) then the timeout mechanism described earlier will detect it.


\subsection{Secure Memory and the \SKMMan{}}
\label{subsec::skmman_mem}

\begin{figure}[htb] 
\centering
\includegraphics[width=0.45\columnwidth]{Figures/secure_memory_map.pdf}
\caption{The secure memory map.}
\label{fig::secure_memory_map}
\end{figure}

To ensure the integrity of the \SKMMan{} we load its code onto a part of the
secure memory region as shown in Figure \ref{fig::secure_memory_map}. Hence,
an attacker that takes control of the main core cannot corrupt the \SKMMan{}. The
\SKM{}, on the other hand, will be loaded onto the main memory (along with the
rest of the kernel)---of course, we will monitor and protect the \SKM{}'s memory
region by the various mechanisms described in this section. 



\subsection{Implementation-Specific Assumptions}
\label{subsec::impl_assumptions}

% \todo[inline]{Collect assumptions here. -- Sibin.}

The primary assumption we make as part of designing this mechanism is that the \SKMMan{} has the ability to access any region in the main memory using physical addresses. Since the \SKMMan{} runs on the SecureCore, which satisfies this requirement, this is not a challenging assumption to discharge.

% \todo[inline]{Anything else in this section? Do we need more subsections here? -- Sibin.}

==> ingress_filtering.tex <==
Links to some useful articles:
\begin{enumerate}
\item IFB example\footnote{https://wiki.gentoo.org/wiki/Traffic\_shaping}
\item Ingress policing and IFB mirroring\footnote{ http://serverfault.com/questions/350023/tc-ingress-policing-and-ifb-mirroring}
\item Explanation redirection vs mirroring\footnote{http://fossies.org/linux/iproute2/doc/actions/mirred-usage}
\item HTB manual \& examples\footnote{http://luxik.cdi.cz/~devik/qos/htb/manual/userg.htm}
\item Classifying packets using tc filters\footnote{http://lartc.org/howto/lartc.qdisc.filters.html}
\item A video on tc classification system\footnote{https://www.youtube.com/watch?v\=cyeJYjZHv5M}
\end{enumerate}
Lessons learned -

==> problem_overview.tex <==
\section{Problem and System Overview}
\begin{itemize}
\item Three classes of traffic
\item Qos requirements - Bandwidth and Delay
\item Focuses on Class 1
\item Problem Statement
\item The big picture as what we are trying to do - Framework (figure) overview with different components and the communication flow among them.\\
- Network Manager - Maintains/obtains details statistics of the networks from the controller\\
- Path Allocation Algorithms with QoS - Routing/Paths layout.\\        ------ Theoretical model to obtain upper bound on end-to-end delay. 
   
- Admission Control
\item Evaluation with network emulator with OVS and real-switches

\end{itemize}

==> skm_API.tex <==
\section{Secure Kernel Module API}\label{sec:skm_API}
